Automating the Generation of Prompts for LLM-based Action Choice in PDDL Planning

Large language models (LLMs) have revolutionized a large variety of NLP tasks. An active debate is to what extent they can do reasoning and planning. Prior work has assessed the latter in the specific context of PDDL planning, based on manually converting three PDDL domains into natural language (NL) prompts. Here we automate this conversion step, showing how to leverage an LLM to automatically generate NL prompts from PDDL input. Our automatically generated NL prompts result in similar LLM-planning performance as the previous manually generated ones. Beyond this, the automation enables us to run much larger experiments, providing for the first time a broad evaluation of LLM planning performance in PDDL. Our NL prompts yield better performance than PDDL prompts and simple template-based NL prompts. Compared to symbolic planners, LLM planning lags far behind; but in some domains, our best LLM configuration scales up further than A$^\star$ using LM-cut.

==> conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

LLMs are rapidly gaining prominence in many sub-areas of AI, and the
question if and how they can be applied in AI Planning is highly
relevant. Following up on previous work in this direction, we show how
to automate the conversion of PDDL into natural language prompts.
Based on this, we contribute broad experiments, highlighting that the
automatic conversion does not result in a performance loss relative to
the previous hand-crafted prompts, and examining performance relative
to representative symbolic methods. The results enhance our knowledge
of LLM action choice performance, and demonstrate convincingly that
LLMs do have \emph{some} action-choice ability, outperforming random
action selection and, in a few cases, even a state-of-the-art optimal
planner. This performance is still far from the state of the art in
symbolic (satisficing) planning, yet it is achieved without any
search, pointing to the potential of more general uses of LLMs in
planning.

The most direct question for future work, in our view, is how to
combine LLMs with symbolic search methods. Our work lays the basis for
that through the automatic translation of PDDL into natural language
prompts, which as our results show boosts the LLM's planning ability.
The space of possible combinations is vast. One could use the LLM to
suggest preferred actions in search, one could search around
LLM-predicted plans or actions, one could apply plan repair to the
LLM's suggestion (as suggested by \cite{valmeekam2023planning} with
LPG \cite{gerevini2003planning}), one could use LLM-generated plans as
the basis for heuristic functions, etc. For further research on the
question whether LLMs on their own (without search) can yield better
planning performance, specialized training or neurosymbolic methods
may be interesting to look at.
%
% Joerg: rewritten after use in search pccured to me as being the most
% direct and promising avenue by far here.
%
%% For future work, it is not clear whether the use of LLMs for action
%% choice, based solely on prompts as explored here, can be brought up
%% to state-of-the-art performance. Specialized training or
%% neurosymbolic methods may be more effective for this purpose. A
%% promising avenue also is to use LLMs not for action choice but for
%% subsidiary functions in plan generation, such as search guidance or
%% dead-end detection.



% Joerg: previous conclusion
%
%% The main contribution of this work is \resourcename\ for automatically converting classical planning benchmarks from PDDL into natural language encodings. %PDDL planning domains are very popular in the classical AI planning research community and available domains differ with respect to a number of characteristics designed to compare the performance classical planning approaches in different settings.
%% In LLM planning experiments on a new suite of 12 planning domains, we find that the planning performance differs considerably between the domains. 

%% By evaluating LLM planners across such a broad range of planning domains, we can pinpoint features of planning problems that make them hard to for LLMs, e.g. plan length and dead-end states. 
%% Enabling LLM planners to handle the combinatorics of such domains, either through better prompts or through the use of neurosymbolic models, is an interesting avenue for future research.

%Our proposed method makes these planning tasks available for research on reasoning and planning with LLMs at a large scale without requiring manual effort or detailed knowledge about PDDL and the domains. Using our \resourcename\ approach we create an initial set of problems from 12 planning domains encoded in NL and test different LLM planning approaches on them. We provide an initial analysis of the performance of the different approaches and of domain-specific and problem-specific factors potentially affecting the performance of LLM planning approaches thereby exemplifying the potential use cases for \resourcename. We hypothesize that \resourcename will be a valuable resource also for other assessment tasks such as the test cases from the PlanBench \cite{valmeekam2023planbench} benchmark and that it support further investigations about the reasoning capabilities of LLMs. 

%Our proposed method allows to run different LLM planning approaches on a variety of different planning domains. 

%testing different LLM planning approaches on classical planning domains at large scale without requiring manual effort and domain experts. While \resourcename\ currently supports only PDDL of limited expressivness the approach could be extended to include more complex operators in the future.

%Available PDDL planning domains differ with respect to a number of characteristics designed to compare the performance classical planning approaches in different settings. Additionally, the complexity of specific problem instances can be easily scaled. Both aspects make them attractive test cases for investigating which characteristics make a planning problem difficult for LLMs and 
%We provide an initial analysis of factors potentially affecting the performance of LLM planning approaches based on the results obtained for the set of NL planning domains created using \resourcename. 

%Our framework currently provides four different planning approaches based on different common prompting strategies. While our experiments focus on comparing different LLM planning approaches we hypothesize that our set of automatically generated NL encodings can be a valuable resource to be used in other approaches investigating the usage of LLMs for planning tasks, including the fine-grained assessment tasks from PlanBench \cite{valmeekam2023planbench}. We provide an initial analysis of what makes specific problems and domains difficult for LLM planners and identify a number of potential characteristics affecting the LLM planning but further research is required to get a better understanding of the challenges for LLM planning approaches. 
 


==> discussion.tex <==
\subsection{Analysis LLM action choice performance}

We observe large differences in the performance of the LLM action choice mechanisms between domains and conduct some initial further analyses of the generated action sequences to get a better understanding of the action choice capabilities of LLMs.

%Overall, the LLM planners perform better on domains with shorter average plan lengths. This could indicate that LLMs are worse at reasoning over long-term interactions or at generalizing from few-shot examples to longer instances.
One factor potentially influencing the action choice performance of LLMs is the plan length, especially since the LLM most often does not have access to the current state in an explicit form but needs to keep track of the state based on the provided NL history. The results from our controlled scaling experiments suggest that there are more factors to it. For the Ferry and Gripper domain, \texttt{ReAct} is able to solve problems with an optimal plan length of more than 50 steps while for Blocksworld already much shorter ones are not solved. These findings match the ones from \citet{silver2022pddl} for Blocksworld and Gripper. Additionally, there is no clear pattern observable between the performance on the scaled Blocksworld data and increasing plan length. In a manual analysis of the predicted action sequences we find that a frequent source of failure is that the LLM predicts actions that stack two blocks on each other that indeed need to be on top of each other in the end but the LLM fails to consider that stacks can only be built from bottom to top.
\dan{I didn't understand this sentence.} \ks{in more technical terms this means that the ``clear'' precondition of stack seems to be the most frequent reason of failure}
This is different in the other three scaled domains where the order in which the different goal facts get satisfied does not matter, i.e. where there are no (sequential) dependencies between the individual subgoals. 
These results suggest that LLMs struggle to reason about long-term dependencies and interactions. %This is in line with findings from \citet{silver2022pddl} who find that LLMs achieve high performance even on large problems of the Gripper domain while they fail on Blocksworld problems where they lack the understanding that stacks need to be build up from the bottom. 
\dan{Wasn't this also one of observations in Rao's papers?} \ks{I was sure I read it there but I couldn't find it anymore in any of the two papers; it seems they do not say it that explicit at least}

We replicate the findings from \citet{liu2023llmp} that GPT-4 is not able to generate correct complete plans in the Floortile domain and we show that even more advanced LLM action choice approaches fail. 
In the Floortile and in the Goldminer domain, for which coverage is low as well, there can be dead-end states, i.e. states from which the goal cannot be reached anymore.
%, because the robots need to paint tiles but cannot move on tiles already painted. Also in the Goldminer domain there can be dead-end states. 
Analyzing the problems not solved with \texttt{ReAct} we find that $92.7\%$ of the unsolved Goldminer and $75\%$ of the unsolved Floortile problems ended in a dead-end state which the LLM action choice was not able to avoid. 

For the Movie domain, \texttt{CoT} and \texttt{ReAct} perform worst. %All optimal plans for problems of this domain have a subsequence of actions in common. However, the interactive planning 
The few-shot examples for both of them differ from all tested problems as they were shortened.
A manual inspection showed that all predicted plans start like the example plan and actions not present in the example get predicted when they are not applicable. This suggests that LLMs have limited capacity to generalize to (the preconditions of) unseen actions. 
Similarly, the few-shot example for the Grippers domain only illustrates picking up a single ball at a time and we observe that the LLM action choice mechanisms very rarely predict action sequences that make use of both grippers. These observations suggest that LLMs are not able to jointly reason over the few-shot examples and the domain description to generalize to other problems.




% FROM PREVIOUS VERSION

%\section{Discussion} \label{sec:discussion}

%In this section, we discuss the results from the experiments in more detail. % in order to get a better understanding of what makes a planning problem or domain difficult for LLM planning. 

%\subsection{Automatic descriptions}\label{sec:dis_encodings}
%The main contribution of our work is the method for to automatically converting PDDL domains and problems into NL descriptions %generate NL encodings of PDDL domains 
%to be used as prompts in %the context of LLM planning and research on the planning and reasoning capabilities of LLMs. Our approach allows to evaluate the action choice performance of LLMs on classical planning domains at a larger scale without requiring costly annotations or domain expertise. 

%When comparing LLM performance on our domain and problem descriptions and on the manual ones from \citet{valmeekam2023planbench} we see a drop in performance for \texttt{CoT} on Blocksworld and \texttt{ReAct} on Logistics. We identified two main differences between the NL descriptions. 

%First, the manual descriptions contain additional information not, or not explicitly, expressed in the PDDL. 
%For example, the manual Blocksworld description states that ``a block is clear if the block has no other blocks on top of it and if the block is not picked up'' although this information is not part of the PDDL definition and hence not included in the automatically generated descriptions. The manual Logistics descriptions explicitly states that the task is ``to transport packages within cities via trucks and between cities via airplanes''. This information is not explicitly included in the PDDL domain but needs to be inferred from the preconditions of the actions. %Additionally, the manual encoding includes the information that there is exactly one truck in each city. This is not even part of the PDDL domain but a convention for the generated problems.

%The second difference concerns the object names. If no types are defined our method assigns names of the form ``object\_x'' whereas in the manual Logistics descriptions each object is assigned a name consisting of its type, e.g.``truck\_0''. The manual Blocksworld names even include colors e.g. ``red block''. 
%While search-based planners are not affected by the names of objects, actions and predicates, LLMs are more susceptible to their semantics \cite{valmeekam2023planning}.

%Any gains in the results for the manual descriptions are likely caused by additional domain knowledge that was added into the on top of the actual domain definition. %This indicates that generating NL encodings of PDDL domains manually is not better \textit{per se}. %Instead, what makes planning with manual encodings slightly easier for LLMs seems to be the amount of external knowledge that an annotator provides to the model for a specific domain. 
%The automatically generated descriptions allow more systematic and fairer comparisons. 

%Overall, we conclude that prompts based on problem and domain descriptions automatically converted into NL by our method leads to comparable action choice performance across different LLM action choice mechanisms and domains.
% of planning problems and domains 
%lead to an comparable planning performance across different planners and domains. 
%Additionally, the overall ranking of the mechanisms and of the domains stays the same.

%\subsection{LLM planning performance}

%Overall, our results support previous claims that LLMs do not perform well on generating correct and directly executable plans for classical planning problems \cite[e.g.][]{valmeekam2023planbench, liu2023llmp}. 

%In line with previous work on reasoning we find that prompting the LLM to reason about the task improves the performance \cite{NEURIPS2022_9d560961}. 
%Also, allowing the LLM planner to correct its predictions based on feedback improves the success rate. However, a ``try-and-error'' approach is often a not feasible way to determine action applicability in the real world due to costs and potential risks. The \Acczero\ results show that LLM planners perform much worse in set-ups where trying out actions and correcting them is not a possible option.

%The interactive LLM planning approaches outperform the random baseline by a large margin. This suggests that LLMs incorporate knowledge that helps them predict better suited next actions than selecting actions at random. Note here in particular that the random baseline selects only from the set of applicable actions whereas the LLM does not have this constraint and each predicted inapplicable action counts towards the step limitation. 

%BFS solves all but one problem within seven minutes and most problems are solved in 10 seconds.
%This shows that even for search-based planning approaches without any heuristic, the specific problems tested in the experiments are easy while many of them are hard for LLM planners. 

%However, the results from the scaling experiments show that for some domains LLM planners can successfully solve planning problems for which BrFS and A* reach the imposed limit. Although the absolute Acc values for BrFS and A* are biased by the specific problems selected, we had no knowledge about whether the LLM planners would be able to solve the larger problems when selecting the test data. Therefore, the results nevertheless clearly indicate the planning problems that LLM planners are able to solve are not simply a limited subset of planning problems solvable by symbolic planners. Further investigating the characteristics of complexity for LLMs compared to symbolic planners in order to identify potential ways to combine their individual strengths is a promising direction of future research.

\begin{comment}
\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{pictures/updated_length_plot.pdf}
    \caption{Number of problems solved per domain (y-axis) plotted against the average optimal plan length of the problems from that domain (x-axis). }
    \label{fig:length_plot}
\end{figure}
\end{comment}


%continue after predicting an non-executable action leads to a higher success rate of reaching the goal state. On the one hand it might not be feasible in many real world tasks to generate a plan in this way as the costs are higher and when trying to execute wrong predicted actions might have bad effects in real tasks. On the other hand, the increase between \Acczero\ and Acc for the interactive LLM planners illustrates that LLMs are capable of recovering and learning from mistakes when being given informative feedback. This is still a desirable ability as not all environments and their rules are fully observable and unforeseen situation can occur. 

%These observations relate to the question of the effect of specific few-shot examples on LLM performance. There have been suggestions for approaches to select few-shot examples for specific tasks \cite[e.g.][]{levy2023diverse} and adopting such an approach is an interesting direction for future investigations (\ks{check the survey paper again}). 

%The positive effect of adding thoughts was largest for the Ferry domain. In the NL encodings, ``(at-ferry ?l)'' got translated to ``?l is at the ferry'' instead of ``the ferry is at ?l'' which was ``fixed'' in the thoughts generated for the planning example. This illustrates that LLMs perform better if actions in a planning domain work similar to the real world, hence matching what they have been exposed to during pretraining.
%While the automatic conversion approach is not guaranteed to generate semantically correct NL encodings, all automatically created NL domain encodings are still consistent within themselves because of the way in which they are composed from the NL fragments.

==> exp.tex <==
\section{Experiments}\label{sec:exp}

We evaluated all our action-choice mechanisms,
\exBasic (Basic), \exCoT, \exAct and \exReAct (ReAct), on different kinds
of input prompts, and against representatives of other planning mechanisms.
We used GPT-4o %\cite{gpt-4o}
as LLM for all evaluated methods. 
%because previous work has shown GTP-4 to be among the
%strongest currently available models for planning
%\cite[e.g.,][]{valmeekam2023planning}.
The LLM policies \exAct and \exReAct are not guaranteed to terminate and
imposing a time limit is not an option here because we use GPT-4o via its API with
high variability of response times.
Therefore, we limit the number of steps for the LLM policies in each
instance by using twice the length of the plan
generated by satisficing greedy best-first search (GBFS) with the FF heuristic
\cite{hoffmann2001ff}.

All results for the LLM-based action choice methods are averaged over 5
runs; each run uses a different value of the ``seed'' parameter
of the GPT-4o API.
%We keep the seed constant for all LLMs involved in the pipeline. \ks{(Not sure whether this is clear enough)} 
We compare our methods with PDDL2NL prompts against the following methods.

%\paragraph{\exManual:}
\exManual:
We compare to the manually provided NL prompts designed by
\citet{valmeekam2023planning} for the domains Blocksworld, Depots and Logistics.

%\paragraph{\exPDDL:}
\exPDDL:
Following the prior work of \citet{silver2022pddl},
we evaluate LLMs taking directly the PDDL input
instead of its NL descriptions.
We use only \exBasic and \exAct as it is not clear how to provide comparable
thoughts for PDDL inputs.
In this case, the {\TLLM} is skipped. Instead, the PDDL action is extracted
from the output of the {\PLLM} using a regular expression and is passed
directly to the simulator.
Additionally, the observations are modified to
``The action \#ACTION\# was successfully executed.'' and
``The action \#ACTION\# is not applicable because \#UNSAT-PRE\#.'' where
\#UNSAT-PRE\# is a concatenation of the unsatisfied PDDL predicates, each
followed by ``is true'' or ``is false''.
For a fairer comparison, we keep a slightly adapted task instruction as part of the
prompts and only replace the NL domain, goal and initial state descriptions
by their original PDDL input (see {\appprompts} for example prompts).
This is closer to the way in which
\citet{valmeekam2023planning} test PDDL inputs as they, in contrast to
\citet{silver2022pddl}, include the PDDL domain description and also a
short task description in natural language.

%\paragraph{\exTemplate:}
\exTemplate:
As a baseline PDDL-to-NL translation, we use a simple template-based method
for converting PDDL into NL prompts:
Unary predicates ``(p ?x)'' are translated to snippets ``\{?x\} is `p''',
higher-arity predicates ``(p ?x1 ... ?xn)'' are translated to
``\{?x1\}, ..., and \{?xn\} are in relation `p''', and PDDL actions
``(act ?x1 ... ?xn)'' are
translated to ``apply the action `act' to object \{?x1\}, ..., and object
\{?xn\}'' where the word ``object'' is replaced with the parameter's type
when it is specified.
The composition of these snippets into the final prompt is done in the same
way as in \resourcename.
Since it is, again, not clear how to provide thoughts for this method, we
use it only with \exBasic and \exAct mechanisms.

%\paragraph{\exRnd:}
\exRnd:
To test whether LLM-based methods carry any information at all, we use a
simple random search (\exRnd) limited by the same number of steps as the
LLM policy that, in every step, selects an applicable action uniformly at
random. The results for \exRnd are averaged over 10 random seeds.
% ten runs with different random seeds.

%\paragraph{\exBFS, \exLMC, \exFF:}
\exBFS, \exLMC, \exFF:
We use breadth-first search (\exBFS) to get a sense of
hardness of tasks and how LLM-based methods compare to a trivial symbolic
baseline.
We also use two strong optimal and
satisficing planner baselines, namely A$^\star$ with the LM-cut heuristic
(\exLMC) \cite{lmcut}, and GBFS with the FF heuristic
(\exFF) \cite{hoffmann2001ff}.
These were run on Intel Xeon
E5-2687W processors with 30 minutes and 8 GB time and memory limits.

We use two benchmark sets.
First, we use 12 classical planning domains (including the three used by
\citet{valmeekam2023planning}; see Table~\ref{tab:coverage}).
In each domain, we generate 21 relatively small
solvable instances with optimal plan lengths between 3 and 20.
We select a small instance (short plan; see details in supplementary
material Appendix~B) for the P-LLM few-shot example (plan
or single action choice), and use the remaining 20 instances as our
benchmarks.

Second, we also compare the best {\resourcename} action-choice mechanisms
to the symbolic baselines (\exRnd, \exBFS, \exLMC, \exFF) on a subset of
IPC benchmarks where it is possible and feasible.
%
First, we disregard domains with PDDL features unsupported by {\resourcename}
(e.g., conditional effects, quantifiers); and since LLM-based methods can rarely scale beyond \exFF (as we show later), we
remove instances that cannot be solved by \exFF within 30 minutes.
Apart from this, the main limiting factor is feasibility in terms of monetary cost for
GPT-4o calls. For 16 domains, the estimated cost (per domain!) was $> 150$USD; for those, we considered only the instances solved by BrFS, reducing the cost to $\leq 150$USD for 15 domains.
%
%\ks{
%\begin{itemize}
%    \item started with 52 benchmarks (+ 1 unsupported PDDL)
%    \item removed 4 (3 domains) because no NL description, 4 (3 domains) because of no thoughts, 1 because smallest plan more than 50 steps, 1 because no single instance solved by \exFF: resulting in 42 we estimated costs for
%    \item removed 28 $> 150$USD, kept 14 benchmarks
%    \item 12 of the remaining were $\leq 150$USD for \exCoT, \exReAct only
%    \item 15 of the finally remaining benchmarks were $\leq 150$USD for \exReAct, \exCoT based on \exBFS
%\end{itemize}
%}
%
In addition to the monetary issues, we could not successfully run our
method on Agricola, Folding, Parking, Richochet-Robots, Sokoban, Tetris,
and Tidybot (e.g., in some cases PDDL2NL failed to generate NL snippets due to large numbers of action parameters).
%
%the following domains.
%In Agricola, Tidybot and Tetris, PDDL2NL failed to generate NL snippets
%with the right number of placeholders and so the final NL description could
%not be generated.
%In Folding, the smallest plan has more than $50$ steps so we did not
%have suitable few-shot examples.
%In Parking, Richochet-Robots and Sokoban,
%our machinery was unable to generate suitable thoughts in
%\exCoT and \exReAct.
%\dan{What exactly is the problem with thoughts?} \ks{we require one thought per action; for examples with long plans the LLM generated less thoughts than required}
%
Overall, the resulting IPC benchmark set consists of 675 instances in 41 domains.







%We ran experiments to evaluate the performance of our LLM action-choice mechanisms on different kinds of input prompts, and against representatives of other planning mechanisms. We next describe the experimental setup, then discuss the results structured into the kind of instances experimented with (non-IPC vs./ IPC).
%
%
%\paragraph{Setup.}
%
%We compare LLM action-choice with our PDDL2NL prompts against (0) the manually provided NL prompts designed by Valmeekam et al.; (1) PDDL prompts rather than
%NL encodings thereof; (2) a simple template-based method to convert PDDL into NL prompts, that we design herefor the purpose of comparison to simpler PDDL2NL methods; (3) random action selection as a
%sanity test; (4) blind breadth-first search as a trivial symbolic
%baseline; as well as (5) strong optimal and
%satisficing planner baselines, namely A* with LM-cut \cite{lmcut} and GBFS with $\hff$ \cite{hoffmann2001ff}.
%
%For comparison (0), we use the three domains provided by Valmeekam et al., Blocksworld, Depots and Logistics. For the other comparisons, our primary experiment extends these benchmarks with another 9 domains, for which we generate smaller instances. This results in a more fine-grained evaluation than IPC instances, due to the limited planning capabilities of LLMs at this point. Specifically, for each domain, we generate 21 solvable instances with optimal plan lengths
%between 3 and 20. We select a small instance (short plan; see details in supplementary
%material Appendix~B) for the P-LLM few-shot example (plan or single action choice), and use the remaining 20 instances as our benchmarks.
%
%For our best action-choice configurations, we also run comparisons (3) (4) and (5) on the original IPC benchmarks. We do so on all domains where that is possible and feasible. The main limiting factor here is feasibility in terms of monetary cost for LLM calls. For 32 pairs of domain and instance suit, running the experiment on all instances solved by GBFS with \hff\ would have resulted in cost $>150$USD (per instance suit!). We ran those domain/instance suits cheaper than this, and we further extended the experiments by domain/instance suits using only those instances solved by breadth-first search.
%
%Apart from monetary cost, we could not run some IPC domains due to technical problems. In Agricola, Tidybot and Tetris, PDDL2NL failed to generate sensible PDDL snippets (e.g.\ for an action schema with 9 parameters); in Folding, the smallest plans had $>50$ steps so we did not have a suitable few-shot example; in Parking, Richochet-Robots and Sokoban, our machinery was for some reason unable to generate suitable thoughts in CoT and ReACT.
%
%
%%Number of removed instances, i.e. where no plan was found by GBFS ff:
%%\begin{itemize}
%%    \item labyrinth23: 14
%%    \item mystery98: 1
%%    \item pipesworld-tankage08: 8
%%    \item scanalzyer08 and scanalyzer11: 2 each 
%%    \item slitherlink23: all 20 removed 
%%    \item snake18: 3 (but domain removed)
%%    \item childsnack14: 3 (but domain removed)
%%    \item depot02: 4 (but domain removed)
%%    \item floortile11 and floortile14: 11 each
%%    \item folding23: 8 (but domain removed)
%%    \item nomystery98: 5 (but domain removed)
%%    \item ricochet-robots23: 5 (but domain removed)
%%    \item sokoban08: 1 (but domain removed)
%%    \item termes18: 1 (but domain removed)
%%    \item tidybot11: 2 (but domain removed)
%%    \item tidybot14: 1 (but domain removed)
%%\end{itemize}
%
%%Removed domains for failure when applying out method:
%%\begin{itemize}
%%
%%    \item agricola: failure generating the NL snippets (wrong formatting, no seed worked); (and smallest plan has length 
%%    $>$ 50)
%%    \item tidybot11 and tidybot14: failure generating the NL snippets, only 2 seeds worked (concerns actions with 9 parameters)
%%    \item tetris14: failure generating the NL snippets, only 2 seeds worked (concerns actions with 6 and 7 parameters)
%%    \item folding23: smallest plan length $>$ 50
%
%
%%    \item and parking14: failure generating thoughts for example with plan length 14 (3 seeds worked)
%%    \item ricochet-robots23: failure generating thoughts for example with plan length 31 (only 4 seeds worked)
%%    \item sokoban08: failure generating thoughts for example with plan length 25 (only 4 seeds worked)
%%\end{itemize}
%%\ks{Failure generating thoughts means that the LLM, that generates the thoughts, does not generate the correct number of thoughts}
%
%%Removed because of other reasons
%%\begin{itemize}
%%    \item storage: PDDL syntax not covered by our approach
%%    \item slitherlink23: 0 coverage of GBFS with ff 
%%\end{itemize}
%
%
%%Removed domains because estimated costs for 5 seeds * 4 approaches larger than 150
%%\begin{itemize}
%%    \item scanalyzer08 (scanalyzer11 was run)
%%    \item transport14 and transport08 (transport11 was run)
%%    \item logistics00 and logistics98 (our own logistics was run)
%%    \item blocks00 (our own blocksworld was run)
%%    \item elevators08 (elevators11 was run)
%%    \item depot02 (our own depot was run)
%%    \item gripper98 (our own gripper was run)
%%    \item visitall11 and visitall14 (our own visitall was run)
%%    \item satellite02 (our own satellite was run)
%%    \item rovers06 (our own rovers was run)
%%    \item barman11 and barman14
%%    \item childsnack14
%%    \item nomystery11
%%    \item pegsol11 and pegsol11
%%    \item parking11 and parking14
%%    \item ricochet-robots23
%%    \item sokoban08 and sokoban11
%%    \item termes18
%%    \item snake18
%%    \item driverlog02
%%    \item tpp06
%%    \item freecell00
%%    \item pipesworld-notakage04
%%    \item pipesworld-tankage04
%%    
%%\end{itemize}
%
%\joerg{standing here. descriptions of exp setup below will eeed to be integrated with the text I now entered above}
%
%%We evaluated our method (both {\PLLM} and {\TLLM}) using the GPT-4 system
%%\cite{openai2023gpt4}
%%as it seems to be the strongest model available nowadays. \ks{adapt}
%% Katharina: this might be a bit misleading: we do not really use GPT-4 for the evaluation per se and we do not directly evaluate our method (and we do not evaluate the T-LLM at all)
%We use GPT-4 \cite{openai2023gpt4} as the \PLLM\ and on few-shot prompting because previous work has shown these to be among the strongest currently available models for planning \cite[e.g.][]{valmeekam2023planning}. We also use GPT-4 as the \TLLM\ and \APBLLM.
%%To limit the financial costs of calling GPT-4, we shortened the examples with
%%thoughts to three steps.
%The LLM policies \exAct and \exReAct are not guaranteed to terminate and
%imposing a time limit is not an option here because we use GPT-4 via its API with
%high variability of response times.
%Therefore, we limit the number of steps for the LLM policies: for each problem the maximum number of steps is set to twice the length of the plan generated by satisficing greedy best-first search with FF heuristic \cite{hoffmann2001ff} (\exFF).
%%24 steps instead (which is at least
%%twice the average of optimal length for all but one domain).
%Since we want to see how well our automatic translations work in comparison to
%the manual ones, we also evaluate all four LLM-based methods on the manual
%descriptions for the Blocksworld, Logistics and Depot domains
%created by \citet{valmeekam2023planning}.
%
%Additionally, we evaluate the LLM-based methods when being provided NL descriptions derived using a simple template-based (\ks{we could also call this rule-based?}) approach for the conversion instead of \resourcename. This baseline conversion translates all PDDL actions into NL snippets of the form ``apply the \#ACTION\# to \#PARAMETERS\#'' where \#PARAMETERS\# is a conjunction of all parameters and their types. For example, ``(drive-truck ?truck ?l-from ?l-to ?city)'' is converted into ''apply the action `drive-truck' to object {?truck}, object {?l-from}, object {?l-to} and object {?city}''. For predicates, we use the template ``\#PRED\# is \#PARAMETER\#'' if there is exactly one parameter, and ``\#PARAMETERS\# are in the relation \#PRED\#'' otherwise. Using these templates,
%``(truck ?truck)'' is converted into ``{?truck} is `truck' '' and 
%``(at ?obj ?loc)'' into ``{?obj} and {?loc} are in the relation `at' ''. 
%
%
%Following the prior work of
%\citet{silver2022pddl},
%we also conduct experiments with LLMs taking directly the PDDL input
%instead of its NL descriptions.
%We use only \exBasic and \exAct as it is not clear how to provide comparable
%thoughts for PDDL inputs. 
%% Katharina: it's possible to use some kind of thoughts (and there is work on other formal languages that does so) but the issue is the comparability here   
%In this case, the {\TLLM} is skipped. Instead, the PDDL action is extracted from the output of the {\PLLM} using a regular expression. % and is passed directly to the simulator. 
%Additionally, the observations are modified to
%``The action \#ACTION\# was successfully executed.'' and
%``The action \#ACTION\# is not applicable because \#UNSAT-PRE\#.'' where \#UNSAT-PRE\# is a concatenation of the unsatisfied PDDL predicates, each followed by ``is true'' or ``is false''.
%For a fairer comparison, we keep a slightly adapted task instruction as part of the
%prompts and only replace the NL domain, goal and initial state descriptions
%by their original PDDL input (see \appprompts\ for example prompts).
%This is closer to the way in which
%\citet{valmeekam2023planning} test PDDL inputs as they, in contrast to
%\citet{silver2022pddl}, include the PDDL domain description and also a
%short task description in natural language.
%
%Lastly, we use several symbolic planning baselines.
%Breadth-first search (denoted as \exBFS) is used to get a sense of
%hardness of tasks and how LLM-based methods compare to a basic uninformed
%search.
%We also compare to two basic state-of-the-art planners:
%optimal A$^\star$ with the LM-Cut heuristic \cite{lmcut} (\exLMC),
%and %satisficing greedy best-first search with FF heuristic \cite{hoffmann2001ff} 
%(\exFF).
%Lastly, to test whether LLM-based methods carry any information at all, we
%use a simple random search (\exRnd) limited by the same number of steps as the LLM policy that, in every step, selects an applicable action uniformly at
%random. The results for \exRnd are averaged over ten runs with different
%random seeds.
%These baselines were run on a cluster of Intel Xeon E5-2687W processors
%with 30 minutes and 8 GB time and memory limits, respectively.

\begin{table}[t]
\centering
{\def\arraystretch{.8}\tabcolsep=1.7pt
{\fontsize{8}{9}\selectfont
\begin{tabular}{l|rrrr|rr|rr||rrrr}
\multirow{2}{*}{Domains}
    & \multicolumn{8}{c||}{LLM-based Approaches} & & & & \\
    & \multicolumn{4}{c|}{\resourcename}
    & \multicolumn{2}{c|}{\exTemplate}
    & \multicolumn{2}{c||}{\exPDDL}
    & \multicolumn{4}{c}{Symb. Baselines}\\
    & \exBasic & \exCoT & \exAct & {\exReAct}
    & \exBasic & \exAct
    & \exBasic & \exAct
    & \exRnd & \exBFS & \exLMC & \exFF \\
\hline
Block.  & 13 & 15  & 17  & \textbf{18} & 8 & 12 & 13 & 14 & 1 & 20 & 20 & 20  \\
\hspace{.2em} $\rotatebox[origin=c]{180}{$\Lsh$}$\exManual & 15 & 14 & 17 & 18 & &  & & & & & &  \\
%\hdashline
Logistics   & 5 & 10 & 16 & \textbf{19}  & 2 & 7 & 6 & 15 & 0 & 20 & 20 & 20\\
\hspace{0.2em} $\rotatebox[origin=c]{180}{$\Lsh$}$\exManual & 3 &5  & 17 & 12 &  & & & & & & & \\
%\hdashline
Depot  & 0 & 5 & 5 & 13 & 0 & 5 & 0 & 3 & 0 & 20 & 20 & 20 \\
\hspace{0.2em} $\rotatebox[origin=c]{180}{$\Lsh$}$\exManual& 3 & 6 & 6 & \textbf{15} & & & & & & & & \\
% \midrule
Ferry  & 7 & 12 & 14 & \textbf{18} & 0 & 13 & 8 & 17 & 0 & 20 & 20 & 20\\
Floortile  & 0 & 0 & 0 & 0 &0 & 0 & 0 & 0 & 0 & 18 & 20 & 20\\
Goldm.  & 1 & 1 & 3 & 1 & 1 & 3 & 1 & \textbf{4} & 0 & 20 & 20 & 20\\
Grid  & 8 & 6 & 16 & \textbf{18} & 1  &  12 &  6& 12 & 0 & 20 & 20&20\\
Grippers  & 9 & 17 & 17 & \textbf{20} & 10 & \textbf{20} & 12 & 19 & 0 & 20& 20& 20\\
Movie  & \textbf{20} & \textbf{20} & \textbf{20} & \textbf{20} & \textbf{20} &\textbf{20} & \textbf{20} & \textbf{20} & 3 & 20&20 &20\\
Rovers  & 0 & 0 & \textbf{18} & \textbf{18} & 1 & 17 & 1 & 11 & 1 & 20& 20& 20\\
Satellite  & 14 & 16 & \textbf{20} & \textbf{20} & 11 & 18 & 14 & 18 & 0 & 20& 20& 20\\
Visitall  & 19 & 19 & \textbf{20} & \textbf{20} &  18&\textbf{20}  & \textbf{20} & \textbf{20} & 8 & 20& 20& 20\\
\hline
$\Sigma$ (240) & 96 & 121 & 166 & \textbf{185} & 72 & 147 & 101 & 153 & 13 & 238 & 240  & 240\\
\hline
\hline
\multicolumn{12}{l}{Further scaled selected domains:} \\
\hline
Block. & 3 & 3 & 12  & \textbf{14} & 0 & 6 & 1 & 4 & 0 & 12 & 19 & 20 \\
Ferry & 0 & 0 & 7 & 15 & 0 & 9 & 0 & \textbf{17} & 0 & 8 & 13 & 20 \\
Gripper & 17 & 12 & \textbf{20} & 19 & 16 & \textbf{20} & 16 & \textbf{20} & 0 & 10 & 8 & 20 \\
Visitall & 9 & 2 & 16 & \textbf{18} & 7 & 17 & 14 & 16 & 1 & 10 & 18 & 20 \\
\hline
$\Sigma$ (80) & 29 & 17 & 55 & \textbf{66} & 23 & 52 & 31 & 57 & 1 & 40 & 58 & 80\\
\end{tabular}
}
}
\caption{\label{tab:coverage}%
Number of solved tasks out of 20 per domain. ``Valm23'' rows show
results of the manual encodings by \citet{valmeekam2023planbench}
in the respective domains.
We show in \textbf{bold} the best LLM-based method.
LLM-based results are averaged over 5 seeds, \exRnd over 10 seeds.}
\end{table}

%\paragraph{Comparison of LLM action-choice methods.}
\paragraph{Comparison to \exManual.}
Table~\ref{tab:coverage} shows the number of solved tasks (coverage) per
domain and overall.
The comparison in Blocksworld, Logistics and Depot to manual descriptions
(see \exManual rows)
shows that using our automatic translations results in
comparable performance.
The most significant difference can be observed for \exCoT and \exReAct
action-choice mechanisms in Logistics where our method solves 5 and 7 more
tasks, respectively.
This is a little bit surprising result considering that the hand-crafted
descriptions by \citeauthor{valmeekam2023planbench} contain additional
information that is not explicitly stated in PDDL
(e.g., that all locations within a city are directly connected)
which is thus not available in the NL descriptions automatically generated
by {\resourcename}.

%\begin{itemize}
%    \item Logistics: automatically generated ones perform better
%    \item for Logistics: problem when driving trucks; drive-truck is not part of the few-shot example; manual descriptions simply states ``Drive a truck from one location to another location.'' as a possible action, not mentioning the city which is left out by the LLM when predicting an action and hence missing for the translation (T-LLM makes one city up then); seems to be more an issue for approaches with thought because city is mentioned in the thought then
%    \item Depot: manual descriptions perform better
%    \item for Depot: no idea why; would need to look into the output files
%\end{itemize}


\paragraph{Comparison between {\resourcename} variants.}
The results of \exBasic with the automatic translation over all
domains support previous findings that a basic prompting technique
does not work particularly well for plan generation
\cite[e.g.,][]{valmeekam2023planbench,liu2023llmp}. Adding reasoning
thoughts (\exCoT) improves performance substantially overall, though
the impact varies per domain and can also deteriorate performance (namely
in the Grid domain).

Using the LLM as an action policy instead of a plan generator in
\exAct yields a major performance boost, dominating \exBasic and
\exCoT consistently in every domain, with major coverage improvements
in many domains. This shows that the use of LLMs, not for plan
generation, but as \emph{a part of plan generation} works much better---in
this case, the LLM being used for action choice only,
with the computation of states being done symbolically and fed back
into the LLM prompts.
%
Adding reasoning thoughts to \exAct in \exReAct yields another
performance boost, consistently dominating coverage across all four
LLM action choice mechanisms (with an exception in Goldminer) and achieving
best LLM performance.

%\begin{itemize}
%    \item automatically generated descriptions perform overall similar to PDDL input
%    \item PDDL overall performs better than using simple Templates for conversion to NL
%    \item still, \exReAct best performing; thoughts for NL are intuitive, but how to get them for PDDL is sth to explore
%    \item seems to be a tendency that domains that for which PDDL works particular well Templates also work well; domains for which automatically generated descriptions work much better then better than both Templates and PDDL 
%    \item PDDL has one advantage in this whole set-up: P-LLM sees exactly the syntax of each action and the generated PDDL action is directly fed into the simulator; i.e. there is no T-LLM involved can make mistake when not being provided the correct number of args, resulting in uninformative feedback (but not sure how to automatically evaluate to what extent this is an issue)
%\end{itemize}

\paragraph{Comparison to \exPDDL and \exTemplate.}
\exPDDL performs slightly better than PDDL2NL for the \exBasic variant,
whereas it is the other way around for \exAct.
Nevertheless, \exReAct with PDDL2NL is clearly superior mainly because it
uses natural sounding, intuitive thoughts in NL.
It is not clear how we could obtain such thoughts for \exPDDL.

%\dan{
%In ECAI paper we wrote:
%
%The comparison to LLM action choice with PDDL input shows that the
%translation to NL is vastly
%superior overall, and is almost consistently beneficial. (A notable
%exception is \exBasic\ in Movie, where significantly more
%tasks are solved with PDDL input than with NL input.) There might be
%superior ways of using \texttt{Act} on PDDL inputs (e.g., using prompt
%engineering, different observations) that are not explored
%here. Nevertheless, our results strongly indicate that LLMs like GPT-4
%tend to work better with NL inputs.
%
%Our automatic PDDL-to-NL translation allows to assess the effect of
%PDDL vs.\ NL input types at a larger scale; and it allows to generate
%the better-performing NL inputs in domain-independent planning,
%providing the basis for deeper combination with symbolic planning
%methods in future work (we list some thoughts in
%Section~\ref{sec:conclusion}).
%}

%\paragraph{Comparison to \exTemplate.}
The simple template-based method (\exTemplate) works decently in some domains
(e.g., Depot, Goldminer, or Visitall), but PDDL2NL generates NL task
descriptions that are at least as good (and often better) in most
domains.
We think this is because LLMs ``understand'' language and therefore
the NL descriptions generated by PDDL2NL are more naturally-sounding than
the \exTemplate descriptions.
In comparison to \exPDDL, \exTemplate is clearly the weaker method.
It also seems that \exTemplate works well in domains where also \exPDDL
works well, and whenever PDDL2NL works significantly better than
\exTemplate, it also works better than \exPDDL.


\paragraph{Comparison to symbolic baselines.}
The comparison to the random baseline \exRnd clearly shows that LLM methods
are able to extract at least some useful information from the task
descriptions (with exception of Floortile where all LLM methods failed).
%This is further supported by the fact that the plans found by \exRnd were on
%average more than twice as long as the plans found by any of LLM methods. \ks{need to recompute plan length!}
%
As can be seen from the \exBFS results, the evaluated tasks are fairly
small, and yet LLM methods fail to solve them all.
The performance of LLM-based methods significantly lag behind symbolic
methods: \exLMC and \exFF solve all tasks, and even
\exBFS solves all tasks except for two in Floortile
(the average runtime of \exLMC, \exFF and \exBFS was
$0.2$, $0.1$ and $6$ seconds, respectively). %\ks{need to recompute runtime?}
%
This behaviour was already observed before---here, we provide a more
comprehensive evaluation enabled by the automatic generation of NL
descriptions.
Nevertheless, we can also see some encouraging results with \exReAct in
many domains.

\paragraph{Scaling experiments.}
To see how far the LLM action choice mechanisms can scale,
we conduct more experiments with larger generated tasks.
We focus on Blocksworld, Ferry, Grippers, and Visitall because \exReAct
performs very well there and it is easy to scale these domains with a
single parameter.

The scaled data for these domains is created as follows.
For each domain, we randomly generate a set of tasks, always varying only a
single parameter: the number of blocks, cars, balls and locations for
Blocksworld, Ferry, Grippers and Visitall, respectively (see \appdom\ for
more details).
Then we run \exBFS and \exLMC on each task with 30 minutes and 8 GB limits.
Then we identify the value $N$ of the varied parameter (e.g.,
number of balls in Grippers) at which either \exBFS or \exLMC is unable to
solve the task.
For the final dataset we select 20 problems per domain for which the scaled
parameter values are around the identified threshold $N$.
We use the same few-shot examples as in the first round of experiments. 
%
%For the Grippers domain, we use only 11 tasks with the largest one including 20
%balls. The reason is that the GPT-4 system has a limit on the number of tokens it
%can process (8~192 tokens) which was already reached by \exReAct on the
%task with 20 balls.
%
The bottom part of Table~\ref{tab:coverage} shows the coverage on the scaled
benchmark set.  
%We can, again, see that NL descriptions usually lead
%to much better performance than PDDL descriptions.  

\exRnd can solve only a single task in Visitall, confirming
the vast superiority of LLM-based methods as much more informed.
%
\exBFS\ is much better, but is also challenged by the size of these
tasks. It is outperformed by \exReAct\ in all domains.
While \exBFS\ is a
very basic symbolic baseline, this provides additional evidence of
\exReAct's planning abilities.
%
Indeed, remarkably, \exReAct outperforms the state-of-the-art
optimal planner \exLMC in 2 domains (and matches its performance in 1).
This is remarkable given that \exReAct,
in contrast to \exLMC, does not perform any search. On the other hand,
it should be noted that Ferry and Grippers are structurally simple
domains, and that \exReAct---in contrast to \exLMC---does not give any
plan-optimality guarantee. 
%
The satisficing planner \exFF, which is comparable to \exReAct\ in
that regard, still has perfect coverage also on these scaled tasks, so
the benchmarks are still not ``hard enough'' to be challenging for
satisficing planning.

Overall, while LLM action choice at this point lags far behind
symbolic planners, there are isolated islands of good performance, and
our results do show promise for LLM planning abilities, in particular
if used as part of a larger symbolic planning machinery (as in case of
\exAct and \exReAct).

% Joerg: needlessly defeatist. 
%
%% The Blocksworld domain is the most complicated domain from the four
%% evaluated here, and \exReAct here lags behind all symbolic methods.

% Joerg: lame
%
%% Nevertheless, we were able to gather this evidence rather easily using
%% our automatic translation method.

\begin{table}[t]
\centering
{\def\arraystretch{.9}\tabcolsep=2.3pt
{\fontsize{8}{9}\selectfont
\begin{tabular}{l|rr|rrrr}
\multirow{2}{*}{Domains}
    & \multicolumn{2}{c|}{\resourcename}
    & \multicolumn{4}{c}{Symbolic Baselines}\\
    & \exCoT & {\exReAct}
    & \exRnd & \exBFS & \exLMC & \exFF \\
\hline
%barman11 (7)  & 0 & 2 & 0 & 7 & 3 &7 \\
%barman14 (3)  & 0 & 1 & 0 & 3 & 0 & 3 \\
barman11/14 (10)  & 0 & 3 & 0 & 10 & 3 &10 \\
blocks00 (35) & 3 & 22 & 0 & 21 & 28 & 35 \\
childsnack14 (16)  & 6  & 15 & 0 & 0 & 0 & 16\\
gripper98 (19)  & 12  & 19 & 0 & 7& 6& 19\\
%logistics98 (2)  & 1  & 2 & 0 & 2 & 2& 2\\
%logistics00 (27)  & 0  & 26 & 0& 10& 19& 27\\
logistics98/00 (29)  & 1  & 28 & 0& 12& 21& 29\\
movie98 (29) & 29 & 29 & 0 & 29 & 29 &  29 \\
rovers06 (6)  & 1  & 5 & 0 &6 &6 &6 \\
satellite02 (5)  & 1  & 4 & 0 &5 &5 &5 \\
%transport08 (11)  & 3  & 8 & 0 & 11&11 &11 \\
%transport11 (20) & 0 & 15 & 0 & 7 & 8 & 20  \\
transport08/11 (31)  & 3  & 23 & 0 & 18&19 &31 \\
%visitall11 (9)  & 5  & 9&0 &9 &9 &9 \\
%visitall14 (4)  & 1  & 4 & 0 & 4& 4& 4\\
visitall11/14 (13)  & 6  & 13&0 &13 &13 &13 \\
\hline
others (482 in 27 domains) & 4 & 18 & 1 & 291 & 311 & 482 \\
\hline
$\Sigma$ (675) & 66 & 179 & 1 & 412 & 441 & 675 \\
%\hline
%data-network18 (19)& 0 & 0 & 0 & 13 & 19 & 19  \\
%elevators11 (20) & 0 & 0 & 0 & 12 & 17 & 20   \\
%floortile11 (9) & 0 & 0 & 0 & 2 & 6 & 9 \\
%floortile14 (9) & 0 & 0 & 0 & 0 & 5 & 9 \\
%ged14 (19) & 3 & 3 & 0 & 19 & 19 & 19 \\
%hiking14 (19) & 0 & 0 & 0 & 12 & 8 & 19  \\
%labyrinth23 (5) &0 &0 & 0 & 5 & 1 & 5 \\
%mprime98 (34) & 0 & 0 & 0 & 20 & 22 & 34  \\
%mystery98 (17) & 0 & 0 & 0 & 14 & 15 & 17  \\
%scanalyzer11 (17) & 0 & 0 & 0 & 9 & 7 & 17  \\
%woodworking11 (20) & 0 & 0 & 0 & 4 & 13 & 20  \\
%zenotravel02 (19) & 1 & 4 & 0 & 7 & 12 & 19  \\
%\hline
% depot02 (17)  & 0  & 3 & 0 & 5& 6& 17\\
% elevators08 (29)  & 0  &0 & 0 & 13 & 19 & 29 \\
% parking11 (19)  & 0  & 0 & 0& 0& 2 & 19 \\
% pegsol08 (29)  & 0  & & 0 & 27 & 26 & 29 \\
% pegsol11(20)  & 0  & 0 & 0 & 18 & 17 & 20 \\
% scanalyzer08 (27)  & 0  & 2 & 0 & 11 & 9 & 27 \\
% transport14 (20)  & 0  & 4 & 0 & 7& 7 & 20\\
% woodworking08 (29)  & 0  & & 0 & 8 & 17 & 29\\
%\hline\hline
%driverlog02 (7)  & 0  &  1 & 0 & 7 &7 &7 \\
%freecell00 (19)  & 0  & 0 & 1 & 19&14 &19 \\
%pipesw.-notank.04 (18)  & 0 & 0&0 &18 & 17&18 \\
%pipesw.tank.04 (13)  & 0 &0 & 0 & 13 & 10 & 13 \\
%snake18 (12)  & 0 & 0 & 0 &12 &6 &12 \\
%termes18 (11)  & 0  & 0 &0& 11 & 5 &11 \\
%tpp06 (5)  & 0  & 0 & 0 & 5 &5 &5 \\
%\hline
%$\Sigma$  & & & & & & \\
\end{tabular}
}
}
\caption{\label{tab:coverage-ipc}%
Number of solved tasks for selected IPC instance suites.
``others'': sum over IPC instance suites where both \exCoT and \exReAct solved less than
25\% of instances.}
\end{table}

\paragraph{IPC benchmarks.}
We also conducted experiments on a subset of IPC domains with the best
plan-generation (\exCoT) and policy (\exReAct) methods (see
Table~\ref{tab:coverage-ipc}).
\exCoT and \exReAct solved less than 25\% in 32 and 27 IPC instance suites,
respectively, and 0 tasks in 29 and 20 instance suites, respectively.
\exCoT solved all tasks solved by \exFF only in movie98, but \exReAct
matched the performance of \exFF in movie98 and gripper98
(and 3 more suites limited to instances solved by \exBFS), and solved only
one less task in childsnack14 and logistics00 (and 2 more suites limited
by \exBFS).
This shows that LLM-based methods are
usually unable to scale to larger instances, but also that there are
domains where \exReAct %the LLM policy with Chain-of-Thought approach, \exReAct,
is able to achieve a good performance.
In fact, it seems that \exReAct either works fairly well or not at all (with
very few outliers).



%%% ---------------------- Discussion Prev Results -------------------%%%
\begin{comment}

\paragraph{Comparison of LLM action choice methods.}
Table~\ref{tab:coverage} shows the number of solved tasks (coverage) per
domain and overall. All results for the LLM-based action choice methods are averaged over 5 runs where for each run we pass a different value to the ``seed'' parameter of the OpenAI API. We keep the seed constant for all LLMs involved in the pipeline. \ks{(Not sure whether this is clear enough)} 
The comparison in Blocksworld, Logistics and Depot to manual descriptions
(see ``Valm23'' rows)
shows that using our automatic translations results in
comparable performance overall. 


Exceptions are 
\exCoT in Blocksworld and \exAct in Logistics where manual
descriptions work significantly better.
The reason might be that the hand-crafted descriptions by
\citeauthor{valmeekam2023planbench} contain additional information that is not explicitly
stated in PDDL (e.g., in their Blocksworld description, it is stated that a
block is clear if no other block is on top of it) and that hence is also not stated in the automatically generated descriptions. 
However, when using the best-performing variant \exReAct the results are
on-par. 


%\paragraph{Comparison between LLM-based methods with \resourcename}
The results of \exBasic with the automatic translation over all
domains support previous findings that a basic prompting technique
does not work particularly well for plan generation
\cite[e.g.,][]{valmeekam2023planbench,liu2023llmp}. Adding reasoning
thoughts (\exCoT) improves performance substantially overall, though
the impact varies per domain and can also deteriorate performance.
%
% Joerg: ue to an oddity in our setup, not the CoT per se. Not needed
% anyway.
%
%% (most significantly in Movie).
%
Using the LLM as an action policy instead of a plan generator in
\exAct\ yields a major performance boost, dominating \exBasic\ and
\exCoT\ consistently in every domain, with major coverage improvements
in many of the domains. This shows that the use of LLMs, not for plan
generation, but as \emph{a part of plan generation} works much better---in
the present case, the LLM being used for action choice only,
with the computation of states being done symbolically and fed back
into the LLM prompts.
%
Adding reasoning thoughts to \exAct\ in \exReAct\ yields another
performance boost, consistently dominating coverage across all four
LLM action choice mechanisms and achieving best LLM performance by far.

%% \dan{Include some discussion from \texttt{discussion.tex}?}

\paragraph{Comparison of input version.}
The comparison to LLM action choice with PDDL input (middle of
Table~\ref{tab:coverage}) shows that the translation to NL is vastly
superior overall, and is almost consistently beneficial. (A notable
exception is \exBasic\ in Movie, where significantly more
tasks are solved with PDDL input than with NL input.) There might be
superior ways of using \texttt{Act} on PDDL inputs (e.g., using prompt
engineering, different observations) that are not explored
here. Nevertheless, our results strongly indicate that LLMs like GPT-4
tend to work better with NL inputs.

\ks{Add templates results here and update based on new results}

Our automatic PDDL-to-NL translation allows to assess the effect of
PDDL vs.\ NL input types at a larger scale; and it allows to generate
the better-performing NL inputs in domain-independent planning,
providing the basis for deeper combination with symbolic planning
methods in future work (we list some thoughts in
Section~\ref{sec:conclusion}).

%This supports previous observations that systems like GPT-4 tend to work
%better with NL inputs, and the automatic PDDL-to-NL translation allowed us
%provide more evidence for it.
% Katharina: I think ''evidence'' is too strong here given that we put almost no  effort in the prompt engineering and observation design whereas we did this for the NL inputs; it's only an indication; and previous work (i.e. Valmeekam) had mixed results for this comparison

\paragraph{Comparison to symbolic baselines.}
The comparison to the random baseline \exRnd clearly shows that LLM methods
are able to extract at least some useful information from the task
descriptions (with exception of Floortile where all LLM methods failed).
This is further supported by the fact that the plans found by \exRnd were on
average more than twice as long as the plans found by any of LLM methods.

As can be seen from the \exBFS results, the evaluated tasks are fairly
small, and yet LLM methods fail to solve them all.
The performance of LLM-based methods significantly lag behind symbolic
methods: \exLMC and \exFF solve all tasks, and even
\exBFS solves all tasks except for two in Floortile
(the average runtime of \exLMC, \exFF and \exBFS was
$0.1$, $0.7$ and $1.7$ seconds, respectively).
%
This behaviour was already observed before---here, we provide a more
comprehensive evaluation enabled by the automatic generation of NL
descriptions.
Nevertheless, we can also see some encouraging results with \exReAct in
Blocksworld, Ferry, Grippers, Movie and Visitall.

\paragraph{Scaling experiments.}

To see how far the LLM action choice mechanisms can scale in domains where it solved all (or
almost all) tasks, we conduct more experiments with larger generated
tasks.  We focus on the Blocksworld, Ferry, Grippers, and Visitall
domains. We leave out the Movie domain for which it is impossible to
generate tasks with longer plans (scaling in this domain essentially
only grows the initial state but the length of plans stays the same). \ks{This motivation doesn't match exactly anymore.}
The scaled data for the four considered domains is created as follows.

For each domain, we randomly generate a set of tasks, always varying only a
single parameter: the number of blocks, cars, balls and locations for
Blocksworld, Ferry, Grippers and Visitall, respectively (see \appdom\ for
more details).
Then we run \exBFS and \exLMC on each task with the same time and memory
limit as in the previous experiments.
For each domain, we identify the value $N$ of the varied parameter (e.g.,
number of balls in Grippers) at which either \exBFS or \exLMC is unable to
solve the task.
For the final dataset we select 20 problems per domain for which the scaled
parameter values are around the identified threshold $N$.
We use the same few-shot examples as in the first round of experiments. 
%
%For the Grippers domain, we use only 11 tasks with the largest one including 20
%balls. The reason is that the GPT-4 system has a limit on the number of tokens it
%can process (8~192 tokens) which was already reached by \exReAct on the
%task with 20 balls.


\begin{table*}[t]
\centering
\caption{Number of solved tasks for selected domains scaled to larger instances. We show in \textbf{bold} the best LLM-based method.}
{\def\arraystretch{.9}\tabcolsep=2.3pt
{\fontsize{8}{9}\selectfont
\begin{tabular}{l||rrrr|rr|rr||rrrr}
\multirow{2}{*}{Domains}
    & \multicolumn{8}{c||}{LLM with} & & & & \\
    & \multicolumn{4}{c|}{\resourcename}
    & \multicolumn{2}{c|}{Templates}
    & \multicolumn{2}{c||}{PDDL}
    & \multicolumn{4}{c}{Symbolic Baselines}\\
    & \exBasic & \exCoT & \exAct & {\exReAct}
    & \exBasic & \exAct
    & \exBasic & \exAct
    & \exRnd & \exBFS & \exLMC & \exFF \\
\hline
Blocks. (20) & 2.6 & 2.6  & 11.6  & \textbf{14.2} & 0.2 & 6.0 & 0.6 & 3.6 & 0.0 & 12 & 19 & 20 \\
Ferry (20) & 0.0 & 0.2 & 6.6 & 14.6 & 0.0 & 8.8 & 0.0 & \textbf{17.4} & 0.0 & 8 & 13 & 20 \\
Gripper (20) & 10.8 & 9.4 & 13.4 & 12.8 & 10.6 & 13.6 & 10.0 & \textbf{15.8} & 0.0 & 11 & 13 & 20 \\
Visitall (20) & 9.2 & 2.4 & 16.0 & \textbf{17.6} & 7.2 & 16.8 & 13.8 & 15.8 & 0.9 & 10 & 18 & 20 \\
\hline
$\Sigma$ (80) &  &  &  &  &  &  &  &  &  & 41 &  63 & 80 \\
\end{tabular}
}
}
\label{tab:coverage-scaled}
\end{table*}


\begin{table*}[t]
\centering
\caption{Number of solved tasks for selected IPC domains.}
{\def\arraystretch{.9}\tabcolsep=2.3pt
{\fontsize{8}{9}\selectfont
\begin{tabular}{l||rrrr||rrrr}
\multirow{2}{*}{Domains}
    & \multicolumn{4}{c|}{LLM with \resourcename}
    & \multicolumn{4}{c}{Symbolic Baselines}\\
    & \exBasic & \exCoT & \exAct & {\exReAct}
    & \exRnd & \exBFS & \exLMC & \exFF \\
\hline
data-network18 (19)& 0.0 &  0.0 & 0.0   & 0.0 & 0.0 & 13 & 19 & 19  \\
elevators11 (20) & 0.0 & 0.0  &  0.0 & 0.0 & 0.0 & 12 & 17 & 20   \\
ged14 (19) & 3.0 & 3.0 & 3.0 & 3.0 & 0.1 & 19 & 19 & 19 \\
hiking14 (19) & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 12 & 8 & 19  \\
movie98 (29) & 28.8 & 29.0 & 29.0 & 29.0 & 0.0 & 29 & 29 &  29 \\
mprime98 (34) & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 20 & 22 & 34  \\
mystery98 (17) & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 14 & 15 & 17  \\
scanalyzer11 (17) & 0.0 & 0.0 & 0.0 & 0.4 & 0.0 & 9 & 7 & 17  \\
transport11 (20) & 0.0 & 0.0 & 7.6 & 15.2 & 0.0 & 7.0 & 8.0 & 20.0  \\
woodoworking11 (20) & 0.0 & 0.0 &0.4& 0.2 & 0.0 & 4 & 13 & 20  \\
zenotravel02 (19) & 0.0 & 0.6 & 1.2 & 3.8 & 0.0 & 7 & 12 & 19  \\
\hline
$\Sigma$  &  &  &  &  &  &  &  &  \\
\end{tabular}
}
}
\label{tab:coverage-scaled}
\end{table*}




Table~\ref{tab:coverage-scaled} shows the coverage on the scaled
benchmark set.  We can, again, see that NL descriptions usually lead
to much better performance than PDDL descriptions.  

\exRnd\ cannot solve any benchmark instance at all here, confirming
the vast superiority of \exReAct\ as a much more informed action
policy.
%
\exBFS\ is much better, but is also challenged by the size of these
tasks. It is outperformed by \exReAct\ overall, which is on-par in
Grippers and much better in Ferry and Visitall. While \exBFS\ is a
very basic symbolic baseline, this provides additional evidence of
\exReAct's planning abilities.
%
Indeed, remarkably, \exReAct is on-par with the state-of-the-art
optimal planner \exLMC in Visitall, and it even solves more tasks than
\exLMC in Ferry and Grippers. This is remarkable given that \exReAct,
in contrast to \exLMC, does not perform any search. On the other hand,
it should be noted that Ferry and Grippers are structurally simple
domains, and that \exReAct---in contrast to \exLMC---does not give any
plan-optimality guarantee. 
%
The satisficing planner \exFF, which is comparable to \exReAct\ in
that regard, still has perfect coverage also on these scaled tasks, so
the benchmarks are still not ``hard enough'' to be challenging for
satisficing planning.

Overall, while LLM action choice at this point lags far behind
symbolic planners, there are isolated islands of good performance, and
our results do show promise for LLM planning abilities, in particular
if used as part of a larger symbolic planning machinery (of which
\exAct\ and \exReAct are basic instances).
    
\end{comment}




==> introduction.tex <==
\section{Introduction}\label{sec:intro}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Large language models (LLMs) have revolutionized a large variety of
%% NLP tasks. An active debate is to what extent they can do reasoning
%% and planning.

%\joerg{I suggest to completely remove the word "AutoPlanBench". It does not capture what we do herem, from a planning community perspective. If you still want to give our pproach/code base a name, you can use "PDDL2NL", maybe "2NL" for short if needed, eg 2NL-LLM instead of APB-LLM.} 

Large language models (LLMs) have revolutionized a large variety of
natural language processing tasks. A recent research trend
investigates whether LLMs can also do planning. The word ``planning''
here is used in a broad sense, encompassing, for example, robot
control \cite{saycan2022i}, text-based games \cite{yao2022react} or
Minecraft \cite{wang2023describe, zhu2023ghost}, but
also less structured tasks such as question answering
\cite[e.g.,][]{NEURIPS2022_9d560961, khot-etal-2021-text}, visual
programming \cite{Gupta_2023_CVPR}, and the orchestration of API calls
\cite{prasad2023adapt}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Prior work has assessed the latter in the specific context of
%% combinatorial planning with PDDL input, based on manually converting
%% three PDDL domains into LLM prompts. 

Here we address PDDL planning. The use of LLMs in this context is, at this stage,
still in its infancy. First works explored what form of input to
provide to the LLM (PDDL, natural language)
\cite{silver2022pddl,valmeekam2023planbench,valmeekam2023planning};
recent work explored the generation of program code for generalized
planning \cite{silver2024generalized}. Here, we follow up on the
prominent work line by \citet{valmeekam2023planbench,valmeekam2023planning}, who
investigated the ability of LLMs to produce plans for PDDL planning tasks. Valmeekam et
al.\ experiment with three wide-spread benchmark domains, Blocksworld, Depots and Logistics, for each of which
they manually engineer natural language (NL) descriptions of the actions
and predicates. They ask the LLM to produce a plan, thus serving as a
form of planner that gives no plan correctness (nor
optimality) guarantee. Valmeekam et al.\ find that LLMs (both GPT-3.5
and GPT-4) are unable to reliably produce correct plans in their 3
benchmark domains, lagging far behind symbolic planning methods.



% Joerg: This distracts from the main storyline here. Describe this in
% experiments when introducing our PDDL variants.
%
%% Comparing the performance when providing the LLM with natural
%% language or with PDDL domain and problem descriptions, they find
%% that GPT-4 performs equally well with natural language and PDDL
%% inputs on the Logistics domain while for Blocksworld using natural
%% language results in a considerable increase in performance.

%% \begin{itemize}
%%     \item \citet{silver2022pddl}: ran LLM planning on PDDL (18 domains) directly (and comparison to random baseline; not sure whether needed for intro already)
%%     \item \citet{valmeekam2023planbench} evaluation framework for assessing LLMs on PDDL planning tasks; initialize their framework with manually converted NL descriptions for two domains: Blocksworld and Logistics
%%     \item \citet{valmeekam2023planning} compare PDDL and NL inputs for GPT-4 and GPT-3.5: for Blocksworld NL performs better, for Logistics comparable results 
%%     \item overall not reliably able to solve traditional planning problems, such as Blocksworld and Logistics
%% \end{itemize}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Here we automate this conversion step, showing how to automatically
%% generate LLM text prompts from PDDL input. 

We extend Valmeekam et al.'s work by automating the conversion of PDDL
into NL prompts for LLM plan generation (and, more
generally, action choice mechanisms, see below). We thus turn the use of LLMs
with NL prompts into domain-independent planning machinery that
does not rely on any input other than the PDDL itself. A key 
challenge here is to ensure that the (syntactic and semantic) relationship
between an action and its arguments is captured correctly, and that
PDDL object types are made explicit in the action descriptions in an
adequate way.

% Joerg: removed some detail to not have to get into the discussion of
% domain-independence of the conversion examples here.
%
We address this by leveraging LLMs themselves to support
the conversion from PDDL to NL. We first use GPT-4o
\cite{gpt-4o} to convert PDDL predicates into NL snippets
based on a few generic conversion examples. We then generate NL
snippets for PDDL action schemas, by first converting the
preconditions and effects based on a simple composition of the
previously generated predicate snippets, and then doing the final
conversion step with an LLM, based again on a few generic examples.
Lastly, we compose the final NL description of the PDDL task for the LLM
prompt from predicate and action snippets together with NL descriptions of
initial state and goal.
%
%\joerg{why was this commented out? please provide brioef explanations
%  to changes in the intro. ... (from a single domain different from
%  the one under translation)}
%% it was commented out becaues it is not correct that the conversion examples come from a single domain; they do not stem from any domain, but each PDDL action and predicate was independently hand-crafted; when we talked about the changes I overlooked that I commented this out 
%
%% We address these challenges by leveraging LLMs themselves to support
%% the conversion from PDDL to natural language. Our approach is
%% in-context, meaning there is no fine-tuning of the LLM and we instead
%% provide a small fixed set of generic conversion examples (hand-crafted
%% once and used domain-independently) to the LLM as part of the input
%% prompt. Specifically, we first use GPT-4 \cite{openai2023gpt4} to
%% convert PDDL predicates into natural language based on a few
%% conversion examples. We then generate natural language descriptions of
%% PDDL action schemas by first converting the preconditions and effects
%% based on a simple composition of the previously converted predicates,
%% and then using again in-context learning based on a few examples for
%% the overall conversion step. Finally, compose the overall
%% domain-description prompt from the predicate and action schema
%% descriptions.
%
%% our method:
%% \begin{itemize}
%%     \item domain-independent prompting-based approach
%%     \item in-context learning: no fine-tuning; instead provide one or more so called few-shot examples to the LLM as part of the input prompt and let it "learn" from the examples only 
%%     \item LLM (GPT-4 \cite{openai2023gpt4}) converts/translates PDDL predicates into natural language in an in-context learning (ICL) set-up based on a small number of hand-crafted conversion examples 
%%     \item then LLM generates a natural language description of a PDDL action including all parameters (and potentially their types) 
%%     \begin{itemize}
%%          \item based on the action name, PDDL parameter specification and schematic natural language encodings of the preconditions and effects 
%%          \item latter one is generated by conjoining the previously generated NL predicate descriptions while inserting the parameter variable names; rule-based composition
%%          \item also based on a small number of hand-written translation examples, i.e. in-context learning
%%     \end{itemize}
%%     \item the action and predicate NL descriptions are the core components needed for describing a domain, a state and a problem
%%     \item rule-based templates that compose the fragments generated by the LLM into adequate natural language descriptions of the domain (consisting of available actions, descriptions of preconditions and effects, as well as type hierarchy)
%%     \item translation examples are designed in a way to enable 1) more flexible and natural language (no restriction to same parameter order in PDDL and NL) and 2) inclusion of object types in referring expressions
%%     \item approach includes heuristic to adapt determiners and guarantee correct coreference resolution 
%% \end{itemize}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% We show empirically that our automatically generated prompts result in
%% similar planning performance as the previous manually generated
%% ones. 
%
Experimenting with the same benchmarks used by Valmeekam et al., we
find that our automatically generated prompts result in
similar performance as the previous manually generated
ones.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Beyond this, we experiment with four different variants of LLM
%% action choice,

%\begin{figure}[t]
%    \centering
%    \includegraphics[width=0.32\textwidth]{pictures/autoplanbench_policy.pdf}
%    \caption{\resourcename\ implements our automatic conversion from
%      PDDL to natural-language prompts, as well as four different LLM
%      action choice mechanisms.}
%    \label{fig:autoplanbench}
%\end{figure}

Beyond this, we provide the first
broad evaluation of LLM performance in PDDL planning, comparing our automatically-generated NL prompts to PDDL prompts and simple template-based prompts, comparing four variants of LLM action choice
mechanisms\footnote{We use ``LLM action choice mechanism''
here as a generic term encompassing both plan generation and action
policies, and to emphasize that (in difference to symbolic planners)
these mechanisms do not use any search, instead choosing actions
directly.}, and comparing LLM planning to several symbolic planning baselines, on a broad range of benchmark domains. 
%
%Figure~\ref{fig:autoplanbench} gives an overview of our implemented framework \resourcename. 

Specifically, we experiment with:
%
\begin{itemize}
\item \textbf{Basic LLM Planning:} Domain and problem description
  provided once, LLM generates a plan. Same as Valmeekam et
  al.\ \cite{valmeekam2023planbench,valmeekam2023planning}.
\item \textbf{CoT LLM Planning:} The LLM also generates a plan,
  but the prompt is enriched by Chain-of-Thought (CoT) prompting
  \cite{NEURIPS2022_9d560961}, asking the LLM to generate
  ``thoughts'' between the predicted actions in the plan.
  \citet{valmeekam2023planning} experimented with a simple version
  of this, producing the states before and after each
  action; here we allow more flexible reasoning, e.g., about the next
  required actions.
\item \textbf{Act:} Here the LLM is used as an action policy instead
  of a plan generator, choosing an individual action for the state at
  each step in the plan. (A similar idea was explored by
  \citet{yao2022react} in non-PDDL-planning contexts.)
  %
  % Joerg: no need to be so elaborate
  %
  %% including question answering, webpage navigation, and a text-based
  %% household environment.
\item \textbf{ReAct:} Inspired by
  \citet{yao2022react}; uses CoT within Act, generating intermediate
  thoughts between actions.
\end{itemize}
%
%% LLM planning approaches:
%% \begin{itemize}
%%     \item test four different, standard prompting approaches for LLM planning / reasoning
%%     \item Basic approach: 
%%     \begin{itemize}
%%         \item standard in-context learning approach where the task description is provided, one in-context example of a problem + solution (here generated plan) and then the LLM generates the solution / plan for the described target problem
%%         \item approach tested by \citet{valmeekam2023planning}
%%     \end{itemize}
%%     \item CoT:
%%     \begin{itemize}
%%         \item \citet{NEURIPS2022_9d560961} introduced Chain-of-Thought prompting (CoT) and showed that it improves performance over basic prompting approaches on a range of reasoning tasks; since then the positive effect of thoughts has been replicated on a large variety of tasks and set-ups
%%         \item main characteristic: LLM is prompted to generate 'thoughts' between the parts that are actually part of the target output (i.e. between the predicted actions for planning)
%%         \item no strict/formal definition of what a thought is: can be anything that relates to intermediate reasoning steps as a human would do to solve a task: e.g. explicitly generating intermediate states, intermediates subgoals, intermediate results; making it explicit what has already been done or what needs to be done next
%%         \item the generation of the thoughts is - in the few-shot setting (i.e. in-context) - elicited by the provided examples which include reasoning thoughts
%%         \item \citet{valmeekam2023planning} also include CoT for Blocksworld (get comparable results) but restrict the 'thoughts' to explicitly generating the current state, action applicabilitiy and resulting state in between any two actions
%%         \item our approach: do not restrict the thoughts but allow more flexible reasoning, e.g. about the next required steps instead of restricting to the state 
%%     \end{itemize}
%%     \item ReAct:
%%     \begin{itemize}
%%         \item ReAct \citet{yao2022react}: combines CoT reasoning with external information from an environment 
%%         \item proposed for interactive decision-making tasks
%%         \item only generate one thought + action at a time
%%         \item get back an observation from the environment it interact with (can in principle be any kind of observation or feedback that gives information about the effect of the action)
%%         \item previous input + LLM output + observation form the input for the LLM for generating the next action 
%%     \end{itemize}
%%     \begin{itemize}
%%         \item Act (also from \cite{yao2022react}): same as ReAct but without generating thoughts
%%         \item only actual difference in the set-up is that in ReAct the few-shot example(s) include thoughts and in Act they do not
%%     \end{itemize}
%%     \item summarize: Basic and CoT only one call to the LLM, Act and ReAct one call per action prediction where input at each step t consists of all previous inputs and outputs of steps 0 to t-1
%% \end{itemize}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% and our automatic machinery enables us to run much larger
%% experiments, providing for the first time a reasonably broad
%% evaluation of LLM action-choice performance in PDDL.
%
Our primary experiment is on 12 domains for which we generate small instances, targeting the relevant scaling range. For a subset of configurations, we also run experiments on all IPC domains, with their original instances, to the extent feasible (monetary cost for LLM calls is the main issue here). We provide
comparisons to (1) LLM action choice based on PDDL prompts
\cite{valmeekam2023planning,silver2022pddl} rather than
NL encodings thereof; (2) a simple template-based method to convert PDDL into NL prompts; (3) random action selection as a
sanity test; (4) blind breadth-first search as a trivial symbolic
baseline; as well as (5) strong optimal and
satisficing planner baselines \cite{lmcut, hoffmann2001ff}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Overall, while LLM action choice at this point lags far behind
%% symbolic planners, our results shed a somewhat more encouraging light
%% than previously suggested. The best LLM configuration soundly beats
%% random action choice, showing that the LLM does carry \emph{some}
%% information about general PDDL planning; in some domains, it scales up
%% further than a state-of-the-art optimal planner.

Compared to the alternative automatic prompting methods (1) and (2), our NL prompts
often yield better performance, in particular as they allow to incorporate Chain-of-Thought (in CoT and ReAct). All four LLM action
choice mechanisms soundly beat (3) random action choice,
%
% Joerg: not needed
%,  Act
%and ReAct do so drastically (5-6 times more instances
%solved overall). 
%
showing that the LLM does carry
\emph{some} information about general PDDL planning (not self-evident given the paucity of internet text about most planning
benchmark domains).%
%
% Joerg: This is not strictly necessary, but let's keep it in for now.
%
\footnote{A similar observation was made by \citet{silver2022pddl},
but in a more limited setting considering PDDL prompts and a set-up
comparable to our Basic LLM Planning configuration, which exhibits
much worse performance than our strongest methods.}
%
The comparisons (4) and (5) to symbolic planners are
less favorable. The satisficing planner (directly
comparable as it does not provide a plan-quality guarantee) reigns
supreme throughout. On the positive side, ReAct outperforms
breadth-first search in 7 domains and the optimal planner in 5 domains.
% ReAct > BrFS in blocks, ferry, gripper, visitall, transport, childsnack, logistics
% ReAct > lmc in ferry, gripper, transport, logistics, childsnack
%
% Joerg: cumbersome
%
%% in Ferry and Visitall domains ReAct outperforms breadth-first search,
%% in Visitall ReAct is on par with the optimal planner, and in Ferry and
%% Grippers domains ReAct outperforms the optimal planner.
%
While these are isolated islands of good performance, they do show
promise for LLM planning abilities, in particular as this performance
is obtained without any search. We will release our code and benchmarks to support further research into the use of
LLMs in PDDL planning.
%
% Joerg: suggest to skip this. Not commony done at icaps
%
%Overall, our contributions are:
%\begin{itemize}
%\item Automating the conversion of PDDL to natural-language prompts.
%\item Showing that this automation does not result in a performance
%  loss relative to the previous hand-crafted prompts.
%\item Implementing four variants of LLM action choice in PDDL
%  planning, transferring ideas previously proposed in different
%  contexts.
%\item Broad experiments on 12 domains and systematically evaluating
%  LLM action choice against representative symbolic planners.
%\item Publicly available code base in \resourcename.
%\end{itemize}

%% The rest of the paper is organized as follows. \joerg{this text par is
%%   optional; we can omit it in case we need space. if it is included
%%   then keep it very simple. just 1 sentence per section.}

% Joerg;: if we incoude such a discussion in the experiments at all,
% this is not something we would emphasize in the introduction unless
% the results are very convincing and striking.
%
%% We conclude with a discussion of the characteristics that make a
%% planning problem difficult to solve for an LLM planner \ks{maybe
%% adapt after revising the discussion} (\S \ref{sec:discussion}).















%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% PREVOIUS INTRO WITH COMMENTS/MATERIAL BY KATHARINA

%% Large Language Models (LLMs) have led to huge improvements on a large variety of NLP tasks. 
%% One active research direction concerns the question whether LLMs can do reasoning and, more specifically, planning.
%% This encompasses both symbolic planning tasks, e.g.\ in robot control \cite{saycan2022i}, text-based games \cite{yao2022react} or Minecraft problem solving \cite{wang2023describe, zhu2023ghost}, but
%% also less structured tasks such as question answering \cite[e.g.][]{NEURIPS2022_9d560961, khot-etal-2021-text}
%% , visual programming \cite{Gupta_2023_CVPR}, and the orchestration of API calls \cite{prasad2023adapt}. 

%% The success of these methods on their respective benchmarks raises the question whether LLMs are actually effective at combinatorially complex tasks such as planning and reasoning or whether existing benchmarks only exercise a simple fragment of the full reasoning task -- after all, LLMs give no correctness guarantees, and they do not perform any search, which was previously thought to be crucial for such tasks. 

%% \begin{itemize}
%%     \item \citet{silver2022pddl}: ran LLM planning on PDDL (18 domains) directly (and comparison to random baseline; not sure whether needed for intro already)
%%     \item \citet{valmeekam2023planbench} evaluation framework for assessing LLMs on PDDL planning tasks; initialize their framework with manually converted NL descriptions for two domains: Blocksworld and Logistics
%%     \item \citet{valmeekam2023planning} compare PDDL and NL inputs for GPT-4 and GPT-3.5: for Blocksworld NL performs better, for Logistics comparable results 
%%     \item overall not reliably able to solve traditional planning problems, such as Blocksworld and Logistics
%% \end{itemize}

%% \citet{valmeekam2023planbench} investigated this question by manually converting a small number of benchmark tasks for classical AI planners, which are specified in the Planning Domain Description Language (PDDL) \cite{pddl1998ghallab}, into natural-language planning tasks for LLMs. They found that LLMs were not reliably able to solve traditional planning problems, such as Blocksworld and Logistics. %such as subgoal interaction.

%% our method:
%% \begin{itemize}
%%     \item domain-independent prompting-based approach
%%     \item in-context learning: no fine-tuning; instead provide one or more so called few-shot examples to the LLM as part of the input prompt and let it "learn" from the examples only 
%%     \item LLM (GPT-4 \cite{openai2023gpt4}) converts/translates PDDL predicates into natural language in an in-context learning (ICL) set-up based on a small number of hand-crafted conversion examples 
%%     \item then LLM generates a natural language description of a PDDL action including all parameters (and potentially their types) 
%%     \begin{itemize}
%%          \item based on the action name, PDDL parameter specification and schematic natural language encodings of the preconditions and effects 
%%          \item latter one is generated by conjoining the previously generated NL predicate descriptions while inserting the parameter variable names; rule-based composition
%%          \item also based on a small number of hand-written translation examples, i.e. in-context learning
%%     \end{itemize}
%%     \item the action and predicate NL descriptions are the core components needed for describing a domain, a state and a problem
%%     \item rule-based templates that compose the fragments generated by the LLM into adequate natural language descriptions of the domain (consisting of available actions, descriptions of preconditions and effects, as well as type hierarchy)
%%     \item translation examples are designed in a way to enable 1) more flexible and natural language (no restriction to same parameter order in PDDL and NL) and 2) inclusion of object types in referring expressions
%%     \item approach includes heuristic to adapt determiners and guarantee correct coreference resolution 
%% \end{itemize}

%% In this paper, we go beyond Valmeekam's work by offering \resourcename\,  an approach that automates the conversion from PDDL problem specifications into natural-language planning problems (Figure~\ref{fig:autoplanbench}). In contrast to Valmeekam's approach, our approach requires no manual effort for extending LLM planning benchmarks to new PDDL domains. This makes it possible, for the first time, to investigate the planning capabilities of LLMs at a larger scale, and it ensures that knowledge that the human problem converter might have about the planning domain does not slip into the planning task. 

%% %In this paper, we go beyond Valmeekam's work by offering \resourcename , a method for automatically converting PDDL problem specifications into benchmarks for LLMs (Fig.~\ref{fig:autoplanbench}). In contrast to Valmeekam's approach, \resourcename\ requires no manual effort for running LLM planning on new domains; the PDDL specification is converted into natural language automatically. This makes it possible, for the first time, to investigate the planning capabilities of LLMs at a larger scale, and it ensures that knowledge that the human problem converter might have about the planning domain does not slip into the natural language task. In addition to the code for converting PDDL into language, we are also releasing an initial data set of natural-language conversions of 12 PDDL domains and of a set of problems for each of them.


%% \begin{figure}
%%     \centering
%%     \includegraphics[width=0.32\textwidth]{pictures/autoplanbench2.pdf}
%%     \caption{\resourcename\ facilitates evaluation of different LLM planners across different domains
%%     by automatically converting PDDL planning tasks.}
%%     \label{fig:autoplanbench}
%% \end{figure}

%% In order to convert PDDL to text at wide coverage, we provide a domain-independent LLM prompting method
%% (\S \ref{sec:method}). The key technical challenge is to ensure that the (syntactic and semantic) relationship between an action and its arguments are captured correctly and that PDDL object types are made explicit in the action descriptions in an adequate way. 

%% LLM planning approaches:
%% \begin{itemize}
%%     \item test four different, standard prompting approaches for LLM planning / reasoning
%%     \item Basic approach: 
%%     \begin{itemize}
%%         \item standard in-context learning approach where the task description is provided, one in-context example of a problem + solution (here generated plan) and then the LLM generates the solution / plan for the described target problem
%%         \item approach tested by \citet{valmeekam2023planning}
%%     \end{itemize}
%%     \item CoT:
%%     \begin{itemize}
%%         \item \citet{NEURIPS2022_9d560961} introduced Chain-of-Thought prompting (CoT) and showed that it improves performance over basic prompting approaches on a range of reasoning tasks; since then the positive effect of thoughts has been replicated on a large variety of tasks and set-ups
%%         \item main characteristic: LLM is prompted to generate 'thoughts' between the parts that are actually part of the target output (i.e. between the predicted actions for planning)
%%         \item no strict/formal definition of what a thought is: can be anything that relates to intermediate reasoning steps as a human would do to solve a task: e.g. explicitly generating intermediate states, intermediates subgoals, intermediate results; making it explicit what has already been done or what needs to be done next
%%         \item the generation of the thoughts is - in the few-shot setting (i.e. in-context) - elicited by the provided examples which include reasoning thoughts
%%         \item \citet{valmeekam2023planning} also include CoT for Blocksworld (get comparable results) but restrict the 'thoughts' to explicitly generating the current state, action applicabilitiy and resulting state in between any two actions
%%         \item our approach: do not restrict the thoughts but allow more flexible reasoning, e.g. about the next required steps instead of restricting to the state 
%%     \end{itemize}
%%     \item ReAct:
%%     \begin{itemize}
%%         \item ReAct \citet{yao2022react}: combines CoT reasoning with external information from an environment 
%%         \item proposed for interactive decision-making tasks
%%         \item only generate one thought + action at a time
%%         \item get back an observation from the environment it interact with (can in principle be any kind of observation or feedback that gives information about the effect of the action)
%%         \item previous input + LLM output + observation form the input for the LLM for generating the next action 
%%     \end{itemize}
%%     \begin{itemize}
%%         \item Act (also from \cite{yao2022react}): same as ReAct but without generating thoughts
%%         \item only actual difference in the set-up is that in ReAct the few-shot example(s) include thoughts and in Act they do not
%%     \end{itemize}
%%     \item summarize: Basic and CoT only one call to the LLM, Act and ReAct one call per action prediction where input at each step t consists of all previous inputs and outputs of steps 0 to t-1
%% \end{itemize}

%% We then empirically establish that on the domains that \citet{valmeekam2023planbench} converted by hand, our automatically converted planning problems yield comparable performance across different LLM planning approaches (\S \ref{sec:exp}). 
%% Finally, we demonstrate the usefulness of our wider-coverage approach by converting 9 further PDDL domains from the planning literature. We evaluate a number of LLM planning approaches on them and compare their performance to symbolic-planning baselines.
%% We find that ReAct backed by GPT-4 \cite{openai2023gpt4} outperforms the other LLM-based approaches and soundly beats the random action selection baseline. Furthermore, we find that for some domains ReAct is able to scale up further than breadth-first search and an optimal SOTA planner.
%% We conclude with a discussion of the characteristics that make a planning problem difficult to solve for an LLM planner \ks{maybe adapt after revising the discussion} (\S \ref{sec:discussion}). We are releasing the code for converting PDDL into language as well as the converted LLM benchmark dataset comprising 12 domains. 

%% \begin{comment}
%% In order to convert PDDL to text at wide coverage, we use a domain-independent LLM prompting method
%% (\S \ref{sec:method}).
%% The key technical challenge is to ensure that the (syntactic and semantic) relationship between an action and its arguments are captured correctly and that PDDL object types are made explicit in the action descriptions in an adequate way. 
%% We then establish that on the domains that \citet{valmeekam2023planbench} converted by hand, our automatic method yields comparable results (\S \ref{sec:exp}). 
%% Finally, we demonstrate the usefulness of our wider-coverage approach by
%% converting 9 further PDDL domains from the planning literature
%% and evaluating a number of LLM planning approaches on them.
%% We find that ReAct backed by GPT-4 \cite{openai2023gpt4} outperforms the other methods,
%% but no LLM planning approach does well on all PDDL domains.
%% We conclude with a discussion of the characteristics that make a planning problem difficult to solve for an LLM planner (\S \ref{sec:discussion}). We are releasing the code for converting PDDL into language as well as the converted LLM benchmark dataset. 
%% \end{comment}



==> limitations.tex <==
\section{Limitations}

%\paragraph{PDDL coverage.} As stated in Section \ref{sec:rel_work} and \ref{sec:method}, \resourcename\ currently only deals with planning domains defined using a subset of the possible operators and features available in PDDL. The approach can be extended further to cover more expressive PDDL. %While these extensions need to be done manually, each will cover not only an additional domain but a theoretically arbitrary large set of planning domains that can be defined with that PDDL version.

%\paragraph{Generalization of results.} 
%All results from the LLM planning approaches are from a single run from GPT-4. Therefore, we cannot draw conclusions on how our results generalize to different LLMs and one-shot planning examples. We chose to focus on few-shot prompts with GPT-4 because previous work has shown these to be the strongest available models for planning. We welcome future research that uses AutoPlanBench to evaluate other LLM planners as well. \ks{mention motivation for GPT-4 in main text; maybe include also 1 other LLM here}
%Additionally, the number of problems tested for each domain is small. However, the focus of this work is on automatically converting PDDL planning domains and problems into NL. % and our experiments show that planning problems converted by \resourcename\ lead to comparable results as problems converted by hand across different LLM planning approaches and domains. 
%While our motivation is to enable investigations of LLM planning capabilities at a larger scale, we do not focus on an comprehensive and detailed evaluation of these capabilities. 

%\paragraph{No correctness guarantees.} 
%The LLM-based approach for converting PDDL into NL has no guarantees that the resulting NL encoding captures the meaning of the PDDL exactly. Nevertheless, all automatically created NL domain encodings are consistent within themselves. This also holds if the encodings for individual actions or predicates are semantically weird such as for the Ferry domain (e.g. ``location\_0 is at the ferry'', see \S \ref{sec:disc_challenges}). This is ensured by the approach that composes the domain encodings from the NL fragments. Furthermore, we show that the automatic NL encodings perform comparable to manual encodings. \ks{Add the consistency characteristic in shorter form to main text.}

%If the \APBLLM\ generates encodings that do not include a placeholder for each of the  parameters in PDDL they cannot be used for the LLM planners because all parameters are required to determine action applicability and state changes. %whether an action is applicable and how the state changes. 

%\paragraph{Thought generation.} The LLM-based approach does not guarantee that the generated thoughts are correct. Additionally, it might happen that the LLM does not generate the required number of thoughts for the example problem, especially when using weaker LLMs. Nevertheless we show that even the automatically generated thoughts improve the performance of LLM planners and can be used for comparative analysis of LLM planners on different domains.

==> mechanisms.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{LLM Action Choice Mechanisms}
\label{sec:mechanisms}

%\subsection{Set-up overview}


\begin{figure}[t]
    \centering
    \includegraphics[width=0.48\textwidth]{pictures/planning_approaches_sketch.pdf}
    \caption{Overview of the set-up for the LLM plan generation and LLM action policy usage.
}
    \label{fig:approach_overview}
\end{figure}

Our automatic PDDL-to-NL translation can be used in concert with
different LLM action-choice techniques.  We distinguish LLM
\emph{planning} techniques (returning a whole action sequence at once)
and LLM \emph{policy} techniques (returning one action at a time).
They both consist of three core components, namely {\PLLM},
{\TLLM} and a simulator (see Figure~\ref{fig:approach_overview}).  The
NL description of the input PDDL task constructed using
{\resourcename} described in Section~\ref{sec:method} is passed to the
LLM (denoted as {\PLLM}) responsible for the actual action choice
(i.e., either a sequence of actions or a single action).  The output
of the {\PLLM} is in the form of NL.  So, we pass its output to
another LLM (denoted {\TLLM}) which translates the NL descriptions of
actions (or action sequences) back to the PDDL format.  Finally, we
pass the PDDL actions returned by the {\TLLM} to the simulator
responsible for validation and analysis of the system's action choice.
We describe each component below.


%The NL planning tasks generated by our conversion methodology can be used in different approaches that incorporate an LLM for generating actions to solve a problem. 
%Here, we experiment with four LLM action choice mechanisms that implement prompting approaches commonly used in research on reasoning and planning with LLMs. \ks{leave this out? somehow I want to make clear that there are more possibilities to use our methods for and that we do not come up with the four ourselves but also don't use them exactly in the same way as done before.}
%Two of the variants use the LLM as a plan generator that generates a complete plan at once (LLM planning). The other two mechanisms use the LLM as an action policy and generates only a single action at a time (LLM policy). The set-ups of both ways of using LLMs for action choice consist of the same three core components as illustrated in Figure \ref{fig:approach_overview}. The set-ups include two LLMs out of which one, the \PLLM, is responsible for the actual action choice and one for translating the NL outputs of the \PLLM\ back into PDDL actions (\TLLM) that are then passed to a simulator that is build on top of a plan validator. We will describe each of the components below.  

\paragraph{Simulator.} 
%
% Joerg: Arrrrrghh!! Environment simulators as a concept are as old as
% the word "AI", and very certainly we're not taking inspiration for
% them in the AI Plannig community from some obscure works in NLP
% working on stuff we would normally not call "planning" at all ...
%
%% Taking inspiration from text-based games such as ScienceWorld
%% \cite{wang2022scienceworld} and AlfWorld
%% \cite{shridhar2021alfworld} used in the context of reasoning and
%% planning with LLMs \cite[e.g.][]{yao2022react, lin2023swiftsage},
%
We implemented an environment simulator for PDDL tasks.
The simulator makes use of the plan validator
VAL\footnote{\url{https://github.com/KCL-Planning/VAL}} to determine
whether an action is applicable in the current state, or to obtain the
unsatisfied preconditions if it is not applicable.  
%
For LLM planning, the simulator only validates the output action
sequence and determines whether it solves the task.
%
For LLM policies, the simulator updates the world state after every
action chosen by the LLM. 

Instead of giving back the resulting world state in PDDL format,
taking inspiration from prior work on non-PDDL forms of planning with
LLMs \cite{wang2022scienceworld,shridhar2021alfworld,yao2022react,
  lin2023swiftsage}, our simulator produces a NL observation about
actions' effects as feedback for the next LLM-policy step.  
%
If the action is applicable, the observation is a statement about the
action being executed (e.g., ``I drive truck truck\_0 from ... to
...'' for the NL action ``Drive truck\_0 from ... to ...'').  This
description is obtained by converting the PDDL action into its NL
description using {\resourcename}.
%
%% ``Drive truck\_0 from location location\_0 in city city\_0 to location location\_1 in the same city'')
%
If the action is not applicable, our simulator states why this is the
case, e.g., ``I cannot drive truck truck\_0 from location location\_0
in city city\_0 to ... because truck\_0 is not at location\_0.''
%
%% ``I cannot drive truck truck\_0 from location location\_0 in city city\_0 to location location\_1 in the same city because truck\_0 is not at location\_0.''.
%
This type of feedback is constructed by converting the PDDL action and
the unsatisfied preconditions into their NL descriptions using the
template ``I cannot \#ACTION\# because \#UNSAT-PRE\#'' where each
\#PART\# is, again, constructed using {\resourcename}. For the creation of grammatical negations of unsatisfied preconditions, %(e.g. ``truck\_0 is not at location\_0'') 
we determine where to add negations based on the position of the auxiliary verb (if there is one) or of the head of the phrase as found by a dependency parser \citep{qi2020stanza}. 
%
% \dan{How exactly do you obtain these justifications? It is also automatically generated, but how?} \ks{added}
% \dan{What simulator? What exactly are you doing here?} \ks{Adapted.}

Lastly, the simulator also determines whether the LLM's action choice
reached the goal which is used as a termination condition for LLM
policies.


\paragraph{\TLLM.} The \TLLM\ translates the NL actions from the \PLLM\
output to valid actions in the PDDL format so that it can be further
passed to the simulator. This translation is done by providing the
\TLLM\ a prompt consisting of a statement providing information about
the task (i.e., translating NL into PDDL) and the output format,
followed by the NL descriptions of all actions of the domain obtained
using {\resourcename} and the objects from the current problem.
Lastly, up to five pairs of an NL action snippet from the domain
and the corresponding PDDL action are included as few-shot examples.
The domain-specific prompts are generated entirely automatically based
on the generated PDDL-to-NL conversions and are identical for all
action choice mechanisms (see \appprompts\ 
%
%% \joerg{reading ``Appendix X'' in a conference submission is
%%   strange. We should excplicitly point to this being in the
%%   supplementary material. So, say ``supplementary material, Appendix
%%   X'' instead}
%
for details).  This approach can be applied to any domain and is
independent of the order of the verb and its arguments in the NL
descriptions, hence allowing more flexibility than the domain-specific,
rule-based translation approach used by
\citet{valmeekam2023planbench}.


\paragraph{\PLLM.} The \PLLM\ component implements the actual action choice
mechanism. 
Figure~\ref{fig:prompt_templates} shows the structure of the prompts for
the \PLLM\ in the LLM planning (left) and LLM policy (right) set-up.
All prompts start with an instruction of the planning task (1), followed by the NL description of %the goal (2) and the domain (3).
the domain (2) and specific instructions for the output of the individual LLM action-choice mechanisms (3).
Then a few-shot example from the same domain is included (4).
It consists of the NL description of the goal of the example problem, the
initial state and an example for the generation of an action or action
sequence---this part is specific for each individual LLM action-choice
method and we discuss it in detail below.
%
%The last part of the prompt consists of specific instructions for the LLM
%action-choice mechanisms (5),
At the end, the goal and initial state of the target
problem~(5) is described (see complete prompts in \appprompts).
%\dan{What is ``general task''?}
%\dan{This few-show example is from the same domain? Where do we get it?}
%\dan{Again, refer to the example in the figure specifically. Which are instructions for LLM planning exactly? Which are ``policy mechanism''? and so on} \ks{I added a first draft of an alternative figure to present them: Figure \ref{fig:prompt_templates}}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.48\textwidth]{pictures/prompts2.pdf}
    \caption{Structure of the prompts for the \PLLM\ in the LLM planning (left) set-up and in the policy set-up at the second prediction step (right). %Prompts consist of (1) a description of the general task, description of the goal (2) and the domain (3), a few-shot example (4) and the planning and policy specific output instruction (5). At the end, the initial state of the target problem is included (6). In the policy set-up, also the history consisting of all previous outputs of the \PLLM\ and the observations is included (7).
    }
    \label{fig:prompt_templates}
\end{figure}

For LLM planning, the \PLLM\ predicts a complete sequence of NL
actions, each in a separate line (see instructions (3)
in~Figure~\ref{fig:prompt_templates} (left)). The output of the
\PLLM\ is translated into PDDL line-by-line by the \TLLM\ and then
passed to the simulator that determines whether the generated action
sequence is a valid plan for the task.

For LLM policies, the \PLLM\ generates a single action that is
directly translated by the \TLLM\ and passed to the simulator which in
turn produces a NL observation (or terminates the planning process in
case the goal is satisfied).  The generated NL observation is added to
the history buffer (see Figure \ref{fig:approach_overview}
(bottom)). In each step, the initial prompt for the \PLLM\ is extended
by all its previous outputs and observations from the history buffer
(see part (6) in~Figure~\ref{fig:prompt_templates} (right)).
%
%%shows the input prompt at the second prediction step, where the first output and the corresponding observation are added below the initial state (7). 
%
This approach provides the LLM access to the history of the action choice
process as LLMs themselves do not include any memory, i.e., each call to an
LLM is independent.
Moreover, the process is not stopped when the \PLLM\ outputs an
inapplicable action as the observations provide information that
can be exploited by the LLM in subsequent steps.
%In the first step, the \PLLM\ generates a thought and an action based on the initial prompt and the simulator produces an observation for the action. The output of the \PLLM\ and of the simulator are appended to the previous input prompt and the extended prompt serves as the input for the next step.
We also equip the {\PLLM} with an option to ask for the current state which is
then provided by the simulator in the form of its NL description.

%For the LLM policy set-up we equip the \PLLM\ with an option to get access to the current states by including the information in the prompt that it can ask for a description of what is currently observable (see Figure \ref{fig:prompt_templates} right, 5). The simulator produces a NL description of the current state as observation when receiving this request.    

%\subsection{LLM action choice methods}\label{sec:appr}

\paragraph{Action choice mechanisms.}
%
The action-choice instructions (part (3)
in~Figure~\ref{fig:prompt_templates}) and few-shot examples (4)
demonstrating the content and format expected from the \PLLM's output
are specific to the individual LLM action-choice mechanisms. We focus
on two LLM planning techniques (Basic and CoT) and
two LLM policy techniques (Act and ReAct), described
in what follows.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.47\textwidth]{pictures/few-shots-all.pdf}
    \caption{Structure of the few-shot examples for the four mechanisms. }
    \label{fig:few-shot_struct}
\end{figure}


%The different behavior of the action choice mechanisms is obtained by the final instructions (Figure \ref{fig:prompt_templates}, 5) in the prompt in combination with the mechanism-specific structures of the few-shot example that is presented in the prompt (4). The few-shot example serves as a demonstration of both the content and the format that the \PLLM\ is expected to generate. Figure \ref{fig:few-shot_struct} shows the structures of the examples for the four variants. 

\paragraph{Basic.} Here, we prompt the \PLLM\ to generate a complete plan of NL actions. We follow \citet{valmeekam2023planning} and present each action of the example plan in a separate line and include a special tag to signal the end of the plan as shown in Figure \ref{fig:few-shot_struct} (top left).


\paragraph{CoT.} \citet{NEURIPS2022_9d560961} showed that
prompting an LLM to generate a chain of thoughts, i.e., a sequence of
explicit reasoning steps, improves the results on a range of reasoning
tasks. The exact form and content of a thought are flexible and can include
explicit reasoning over the current state, the next action or a goal
to satisfy. For example, a thought in Logistics could be ``Now,
package\_0 is at truck\_1 and truck\_1 is at location\_2
in city\_4. Package\_0 needs to be moved to location\_3 in city\_4.''
The generation of thoughts by the \PLLM\ is elicited by adding thoughts
between the actions in the \Pex\ (see Figure \ref{fig:few-shot_struct},
bottom left) and additional instructions in the prompt (see part (3) in~Figure~\ref{fig:prompt_templates}).

\paragraph{ReAct.} ReAct combines CoT reasoning with information received
from an environment.
It was originally proposed for interactive decision-making tasks \citep{yao2022react}.
% \dan{missing citation? If we don't want to cite, remove the sentence.}.
At each step, the \PLLM\ predicts a thought and an action and receives an observation from the simulator (see Figure \ref{fig:few-shot_struct}, bottom right). 
The complete output of the \PLLM\ including the thought and the
observation are added to the history buffer. % for the prompt at the next prediction step. 
%As the length of the input increases with each step, the few-shot example does not demonstrate all individual steps but the last input (including the complete history) and output (see Figure \ref{fig:few-shot_struct}, bottom right). %In order to demonstrate which parts the \PLLM\ is supposed to generate, LLM outputs are preceded by the tag ``You:'' and parts provided by the simulator by ``I:'' in the few-shot examples. 

\paragraph{Act.} The Act mechanism works in the same way as ReAct but does not include reasoning thoughts (Figure \ref{fig:few-shot_struct}, top right). 


%\paragraph{Few-shot example generation.}
Note that all \Pex s are generated automatically by converting one small example
problem and its plan into NL. For the LLM policy mechanisms, the simulator is used to generate the corresponding observations. 
%
For CoT and ReAct, reasoning thoughts are required. % for the \Pex s.
%\dan{I don't understand the following sentence:}
We use an LLM-based approach to obtain them: first the \Pex\ in the ReAct structure is created (Figure \ref{fig:few-shot_struct}, bottom right), but with placeholders instead of actual thoughts.
We manually create thoughts for one example problem from Logistics and use this as few-shot example when prompting
an LLM to come up with appropriate thoughts to replace the placeholders for
other problems and domains. For the CoT \Pex s the observations get removed afterwards (see \appreact).


==> method.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.48\textwidth]{pictures/conversion_example.pdf}
% TODO: Remove for CR
\setlength{\abovecaptionskip}{-.3ex}
\setlength{\belowcaptionskip}{-2ex}
    \caption{Part of the prompt for converting PDDL predicates into NL consisting of the task description (top), few-shot examples (middle) and the target predicate (bottom). }
    \label{fig:conv_prompt}
\end{figure}



\section{Converting PDDL into Natural Language}\label{sec:method}


We contribute an automatic conversion, \resourcename, of PDDL domains and problems
into NL descriptions.
%
Our method first produces PDDL-to-NL mappings for objects, predicates, and actions, then joins these together into a prompt tasking the LLM to
solve the described planning instance. To achieve this automatic conversion, we leverage an LLM
(called \APBLLM, short for \resourcename-LLM), with few-shot
prompting on generic examples (fixed once and used for any input PDDL)  for each part of the conversion.
%and few-shot prompting, which we refer to as
%\APBLLM\joerg{Why ``APB''? This sentence is very unclear to me. What
%  is ``the'' few-shot prompting method? Is there exactly one such
%  method? Why do we introduce an acronym for LLM+fewshotprompting at
%  all?}.


%\begin{table*}[ht]
%\caption{Examples of the LLM-based conversion of PDDL (Input) predicates of the Logistics domain (top) and the ``drive-truck'' action (bottom) to NL descriptions (Output). Tokens in curly brackets serve as placeholders for the objects when constructing the domain and problem NL descriptions.}
%    \centering
%    %\small
%    \begin{tabular}{|l|l|l|l|l|}
%    \hline
%         Input: & (truck ?truck ) & (location ?location) & (at ?obj ?loc) & (in-city ?obj ?city)\\
%         \hdashline
%         Output: & \{?truck\} is a truck & \{?location\} is a location &
%          \{?obj\} is at \{?loc\} & \{?obj\} is in the \{?city\}\\
%         \hline\hline
%         Input: & \multicolumn{4}{|l|}{action: drive-truck} \\
%         & \multicolumn{4}{|l|}{parameters: (?truck ?loc-from ?loc-to ?city)}\\
%         & \multicolumn{4}{|l|}{preconditions of drive-truck: ?truck is a truck and ?loc-from is a location and ?loc-to is a location and ?city is a city} \\
%         & \multicolumn{4}{|l|}{\qquad \qquad \qquad and ?truck is at ?loc-from and ?loc-from is in city ?city and ?loc-to is in city ?city} \\
%         & \multicolumn{4}{|l|}{effects of drive-truck: it becomes true that ?truck is at ?loc-to and it is not the case anymore} \\
%         & \multicolumn{4}{|l|}{\qquad \qquad \qquad that ?truck is at ?loc-from}\\
%         \hdashline
%         Output: & \multicolumn{4}{|l|}{drive truck \{?truck\} from location \{?loc-from\} in city \{?city\} to location \{?loc-to\} in the same city}\\
%    \hline
%    \end{tabular}
%    
%    \label{tab:pddl2text}
%\end{table*}

Figure \ref{fig:conv_prompt} illustrates the input prompt received by the
{\APBLLM} for translating PDDL predicates into NL.
The prompt consists of three parts.
The first part is a manually designed instruction explaining the PDDL-to-NL translation.
The second part consists of several examples illustrating to the {\APBLLM} how
to conduct the translation.
These so-called few-shot examples are hand-crafted, but we use exactly the
same examples independently of the target PDDL domain.
We use seven examples of predicates of arity ranging from 0 to 2.
After the examples, we pass the actual predicate that we want to translate\footnote{We use \#PART\# to mark parts of the shown prompts that
are placeholders for actual content omitted for the presentation throughout
the paper.} to the LLM, 
%The last part of the prompt consists of the actual predicate that we want
%to translate
i.e., we tell the {\APBLLM} which PDDL predicate we want to
translate to NL (e.g., we provide ``(at ?x ?y)'' as input)
and expect the {\APBLLM} to return its NL description (e.g.,
``\{?x\} is at \{?y\}''). 
Table~\ref{tab:pddl2text} (top) shows the NL descriptions of predicates
generated in the Logistics domain.
Note that the NL descriptions are constructed as \textit{snippets} with
placeholders for actual objects (e.g., ``\{?obj\}'') which are replaced later
when constructing the final NL task description.
Therefore, we require the LLM to generate snippets that include all variable names from the PDDL, each surrounded by brackets. We automatically check whether this condition is met and if not the \APBLLM\ is prompted once to revise the previous output. 

NL snippets of actions are generated analogously using a similar
prompt with different examples.
In this case, each example consists of the name of the action, its parameters, and NL descriptions of the
preconditions and effects that are constructed using the NL snippets of the predicates generated by the \APBLLM\ as described above.
%\APBLLM's translation of predicates described above.
The precondition is constructed by joining NL descriptions of
its positive atoms by ``and'' and the conjoined negative preconditions are preceded by ``it is not the case that''. The NL descriptions of the positive (add) and negative (delete) effects are conjoined analogously.
%and similarly for effects where we also
%distinguish positive (add) and negative (delete) effects. 
Moreover, we compile away parameter types using unary predicates
\cite[e.g.,][]{helmert2009concise}. %that are also translated to NL using {\APBLLM}.
We use the same four hand-crafted few-shot examples of actions independently of the target domain. As for predicates, snippets not matching the formal requirements are revised once. % by the \APBLLM. 
%(again, the same ones independently of the target PDDL domain).

\begin{table}[t]
    \centering
{\def\arraystretch{1}\tabcolsep=2.3pt
    \small
    \begin{tabular}{|l|l|l|}
    \hline
         In: & (truck ?truck ) & (location ?location) \\
         \hdashline
         Out: & \{?truck\} is a truck & \{?location\} is a location \\
         \hline
         In: & (at ?obj ?loc) & (in-city ?obj ?city)\\
         \hdashline
         Out: & \{?obj\} is at \{?loc\} & \{?obj\} is in the \{?city\}\\
         \hline\hline
         In: & \multicolumn{2}{|l|}{action: drive-truck} \\
         & \multicolumn{2}{|l|}{parameters: (?truck ?l-from ?l-to ?city)}\\
         & \multicolumn{2}{|l|}{preconditions of drive-truck: ?truck is a truck and } \\
         & \multicolumn{2}{|l|}{\qquad ?l-from is a location and ?l-to is a location and  } \\
         & \multicolumn{2}{|l|}{\qquad ?city is a city and ?truck is at ?l-from and ?l-from} \\
         & \multicolumn{2}{|l|}{\qquad  is in city ?city and ?l-to is in city ?city} \\
         & \multicolumn{2}{|l|}{effects of drive-truck: it becomes true that ?truck is at ?l-to} \\
         & \multicolumn{2}{|l|}{\qquad and it is not the case anymore that ?truck is at ?l-from} \\
         \hdashline
         Out: & \multicolumn{2}{|l|}{drive truck \{?truck\} from location \{?l-from\} in city }\\
                 & \multicolumn{2}{|l|}{\qquad \{?city\} to location \{?l-to\} in the same city}\\
    \hline
    \end{tabular}
    
}
\caption{\label{tab:pddl2text}%
Example PDDL-to-NL translation by the {\APBLLM} in the Logistics domain;
predicates at the top; the ``drive-truck'' action at the bottom.}
\end{table}

Table \ref{tab:pddl2text} (bottom) shows an example translation of the
``drive-truck'' action from the Logistics domain.
It illustrates two interesting characteristics of our NL snippets.
First, the
order of the arguments in the generated NL snippet can deviate from the
order of the parameters in the input PDDL domain.
The order of parameters can be
arbitrary and might not match a natural sounding or even syntactically
correct order of arguments of the action verb in NL. We therefore include
one few-shot example where the order deviates in the prompt for the
\APBLLM\ to prevent the LLM from inferring that the order needs to be
identical.
%
Second, the generated NL snippet of ``drive-truck" states the type of
each parameter, i.e., it makes use of the information
from preconditions to infer appropriate types. The complete conversion prompts can be found in \appapb.
%\footnote{All appendices can be found in the supplementary material.}
% removed footnote as all references to the appendices explicilty state the supplementary material now


\begin{comment}
\begin{figure}[ht]
\subfloat[NL description of the Logistics domain, consisting of the available actions with parameters ($\mathcal{A^{PA}}$), their preconditions ($\mathcal{A^{PR}}$) and effects ($\mathcal{A^E}$) as well as the type hierarchy ($\mathcal{T}$).]{\includegraphics[width=0.48\textwidth]{pictures/nl_domain_ex.pdf}\label{fig:nl_domain}}
    \par\bigskip
\subfloat[NL description of a Logistics problem stating the goal ($\mathcal{G}$), the available objects ($\mathcal{O}$) and the initial state ($\mathcal{I}$).]{\includegraphics[width=0.48\textwidth]{pictures/problem_nl.pdf}\label{fig:nl_problem}}
    \caption{Excerpt from the NL descriptions generated by \resourcename\ (\ref{fig:nl_domain}) for the PDDL shown in Fig. \ref{fig:domain_ex}.}
    \label{fig:domain_ex_nl}
\end{figure}
\end{comment}

%The ``drive-truck'' action in Table \ref{tab:pddl2text} illustrates two interesting characteristics of the NL encodings resulting from the way in which our conversion method works. First, the order of the arguments in the generated NL encoding can deviate from the order of the parameters in PDDL. The order of PDDL parameters can be arbitrary and might not match a natural sounding or even syntactically correct order of arguments of the action verb in NL. We therefore include one few-shot example where the order deviates in the prompt for the \APBLLM\ to prevent the LLM from inferring that the order needs to be identical. 
%
%Second, the generated NL description of ``drive-truck" states the type for each parameter. This illustrates that the LLM makes use of the information in the preconditions to infer appropriate types. 


With the NL descriptions of predicates and actions
in the form of snippets, we proceed with the generation of the domain
and problem NL descriptions of the input PDDL task.

Figure \ref{fig:nl_domain} shows an excerpt from the NL \emph{domain} description of the
PDDL Logistics domain (Figure~\ref{fig:pddl_domain}).
NL domain descriptions are designed to include the same information as the
input PDDL.
They start with the description of all possible actions ($\mathcal{A^{PA}}$),
followed by their preconditions ($\mathcal{A^{PR}}$) and effects
($\mathcal{A^{E}}$). If the domain is typed, a verbalization of the type
hierarchy is added also ($\mathcal{T}$). Our template takes care
of the statements introducing each part of the prompt (e.g. ``I can carry
out the following actions:'') as well as of adequately composing the
preconditions and effects into NL sentences (e.g. ``Once I \#ACTION\# it is
not the case anymore that \#EFFECT\#'' for delete effects). The positive
and negative preconditions are presented in two individual sentences. The
same applies to the add and delete effects.
Moreover, we use a heuristic to add
indefinite determiners to ensure that the domain encodings refer to objects
in general instead of specific objects (e.g. ``drive \textbf{a} truck A'')
and that the referring expressions allow to correctly infer which
expressions refer to the same object. %coreference resolution.
%\subsection{NL domain and problem descriptions}

%\paragraph{Domain descriptions.}
%
%The NL descriptions of the PDDL domains are composed based on the domain-specific NL predicate and action descriptions using a domain-independent template-based approach. Figure \ref{fig:nl_domain} shows an excerpt from the NL Logistics domain description. All NL domain descriptions include exactly the same information as the PDDL domains: they start with the description of the possible actions ($\mathcal{A^{PA}}$), followed by all preconditions ($\mathcal{A^{PR}}$) and all effects ($\mathcal{A^{E}}$). If the domain is typed, a verbalization of the type hierarchy is added at the end ($\mathcal{A^{T}}$). The template takes care of the statements introducing each part of the prompt (e.g. ``I can carry out the following actions:'') as well as of adequately composing the preconditions and effects into NL sentences (e.g. ``Once I \#ACTION\# it is not the case anymore that \#EFFECT\#'' for delete effects). The positive and negative preconditions are presented in two individual sentences. The same applies for the add and delete effects. We use a heuristic to add indefinite determiners to ensure that the domain encodings refer to objects in general instead of specific objects (e.g. ``drive \textbf{a} truck A'') and that the referring expressions allow to correctly infer which expressions refer to the same object. %coreference resolution. 
%%\dan{What's ``coreference resolution''?} \ks{Is this explanation enough?}


\begin{comment}
\begin{figure}[]
    \centering
    \includegraphics[width=0.49\textwidth]{pictures/nl_domain_ex.pdf}
    \caption{Excerpt from the generated NL description of the typed logistics domain, consisting of the available actions (1), their preconditions (2) and effects (3) as well as the type hierarchy (4).}
    \label{fig:domain_descr}
\end{figure}
\end{comment}

%\paragraph{Problem descriptions.} As shown in Figure \ref{fig:nl_problem}, the NL problem descriptions consist of the same information as the PDDL problem files: the descriptions of the goal state ($\mathcal{G}$), the available objects with their types ($\mathcal{O}$) and the initial state ($\mathcal{I}$). 
The NL \emph{problem} descriptions (see example
in~Figure~\ref{fig:pddl_prob} and \ref{fig:nl_problem})
specify the goal condition ($\mathcal{G}$),
available objects with their types ($\mathcal{O}$), and the
initial state ($\mathcal{I}$).

%As described in Section~\ref{sec:rel_work}, PDDL problem files define the available objects, the initial state and the goal conditions. Our generated NL problem descriptions include exactly the same information encoded as follows (see Figure \ref{fig:nl_problem}). 

The object names in PDDL problems can be any strings of characters and they
often consist of single letters and numbers. For the NL description of the
planning problems, more natural and semantically related object names are desirable. 
Our method generates new object names based on their types. If a domain is typed, we name each object after its (most specific) type and enumerate them, e.g. ``t0'' (Figure \ref{fig:pddl_prob}) becomes ``truck\_0'' (Figure \ref{fig:nl_problem}). Otherwise, we use the most general PDDL type ``object'' for all object names. 

% Comments
%\dan{Example actually shows ``obj\_'' not ``object''} \ks{yes, but the domain is typed and therefore the type is used for the name and not ``object''; and ``obj'' is the type from the type hierarchy; Update: I changed the examples in Figure 2 and Figure 3} 
%\dan{Also, refer specifically to Figure~3b} \ks{added}

The NL descriptions of the initial state and goal are constructed using the
NL descriptions of the corresponding predicates
obtained by the {\APBLLM}.
For example, the goal ``(at p0 l0-0)'' (Figure \ref{fig:pddl_prob}) is converted into ``package\_0 is at
location\_0'' and appended to ``My goal is that in the end'' (Figure
\ref{fig:nl_problem}). If there is more than one goal fact, they are
conjoined using ``and''. The description of the initial state is
constructed analogously but starts with ``Currently,''. % instead of ``My goal is...''.
%The initial state and the goal of a PDDL problem are defined by the set of predicates that are or need to be true respectively. The NL descriptions of both are therefore derived based on the NL descriptions of these PDDL predicates and the converted object names. For example, the goal ``(at p0 l0-0)'' (Figure \ref{fig:pddl_prob}) is converted into ``package\_0 is at location\_0'' and appended to ``My goal is that in the end'' (Figure \ref{fig:nl_problem}). If there is more than one goal fact, they are conjoined using ``and''. The description of the initial state is constructed analogously but starts with ``Currently,'' instead of ``My goal...''. 
%A world state is defined by the set of all atoms that are true in it. The initial state is therefore described as a concatenation of the NL predicate descriptions defining the state where the objects are referred to by the adapted object names. %Likewise, the goal conditions are encoded based on the NL descriptions of the goal predicates and the object names.  
%The NL goal descriptions are derived in the same way.
% \dan{I didn't get this description. Refer to the previous section where the predicate translation is described and use examples (e.g., (at obj\_0 location\_0) is translated to ``obj\_0 is at location\_0''). More precisely describe how we construct goal (``My goal is that in the end...''), how we construct the initial state (``Currently, ...'').} \ks{Adapted}

% Previous version
\begin{comment}
We use an LLM-based approach to generate the mappings based on a small number of hand-crafted few-shot examples (see Appendix \ref{app:apb} for the prompts). % and will refer to the LLM for the PDDL-to-text generations as \APBLLM\.
\dan{"see Appendix C" needs to be re-phrased because appendices are not
part of the publication -- for submission we need to refer to supplementary materials, but for CR it would be best if we cite it}\ks{ K: so how exactly should the reference to appendices look like?}
We manually create seven examples of PDDL predicates with zero, one or two parameters and four examples of actions with one to three parameters. For each of the PDDL examples we manually construct NL descriptions and use these example pairs for all conversions.

First, we use the LLM (\APBLLM) to separately translate each PDDL predicate into NL. %The prompt for this step includes seven hand-written examples of predicates in PDDL and possible NL encodings for them. 
\dan{What is \APBLLM?} \ks{K: just a name to differentiate the LLM used for generating the conversions (AutoPlanBench LLM) from the LLMs used for action choice and translating back; I'm happy to use a different name for it}
Table \ref{tab:pddl2text} (top) shows the NL fragments generated by the \APBLLM\ for predicates from the Logistics domain. The fragments are templates because - as in PDDL - the parameter tokens are placeholders for the actual objects. 

In the next step, the descriptions for the actions get generated in the analogously using a similar prompt but with few-shot examples of actions instead of predicates.
%\dan{Not actually the same way. ``Analogously''?}
 We provide the complete information from the action scheme in the PDDL domain file, as shown in Table \ref{tab:pddl2text} (bottom).
\dan{What do you mean by ``complete information from the action scheme''.
This needs to be clarified.}
 The preconditions and effects are presented as natural language sentences that are composed by conjoining the previously generated predicate descriptions based on templates. %The lower part of Table \ref{tab:pddl2text} presents the input and generated output for the ``drive-truck" action. 
For the generation of the NL descriptions, we convert the PDDL action definitions from typed into untyped PDDL to include the type constraints as preconditions.
\dan{How exactly? Can you point to the example? Here we could probably even
cite ``Helmert: Concise Finite Domain Representation...''} %\ks{K: I add the ``parameter\_name is a type\_name'' to the preconditions and remove the types for the conversion}

Providing the preconditions and effects improves the correctness of the outputs as it helps the LLM to determine the semantic roles of the parameters.
\dan{``Improve correctness'' is not accurate -- correctness does not have
degrees. ``improve accuraccy of the
translation''?} 
For example, ?l1 and ?l2 are equally good variable names as ?loc-from and ?loc-to in PDDL but do not allow to infer which is the start location and which the destination.
%\dan{start -> start location?}
 The roles become clear when adding the information that e.g. ?l1 is the location where the truck needs to be (precondition) and ?l2 the location where it will be afterwards (effect).  
\dan{``needs to be'' is a little bit confusing. ``needs to be in order to
be able to execute the action'' which is probably unnecessarily long.}

The example of action ``drive-truck'' in Table \ref{tab:pddl2text} illustrates two interesting characteristics of the NL encodings resulting from the way in which our conversion method works. First, the order of the arguments in the generated NL encoding can deviate from the order of the parameters in PDDL. The order of PDDL parameters can be arbitrary and might not match a natural sounding or even syntactically correct order of arguments of the action verb in NL. We therefore include one such PDDL-NL pair as example in the prompt for the \APBLLM\ to prevent the LLM from inferring that the order needs to be identical. 

Second, the generated NL description of ``drive-truck" states the type for each parameter. This illustrates that the LLM makes use of the information in the preconditions to infer appropriate types. %In order to get the same behavior for typed and untyped domains, we convert the action definitions into untyped PDDL by . 
%\dan{``indicates'' does not sound right to me. ``This allows LLM to make use...''?}

\dan{We also need to somehow argue how we decided for those particular examples
and not for others.} \ks{K: not sure how to argue for the decisions, I simply hand-crafted a few simple examples (with the exception of one action example where I deliberately switched the order of arguments in PDDL and NL)}
\end{comment}


==> relatedwork.tex <==
\begin{comment}
\begin{figure*}
    \centering
        \begin{subfigure}[b]{0.48\textwidth}
        \includegraphics[width=\textwidth]{pictures/domain_pddl.pdf}
        \caption{PDDL domain definition including a subset of the state predicates (blue) and the ``drive-truck'' action (orange). The typed version includes the type hierarchy (green).}
        \label{fig:pddl_domain}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.48\textwidth}
        \includegraphics[width=\textwidth]{pictures/nl_domain_ex.pdf}
        \caption{Generated NL description of the typed logistics domain, consisting of the available actions (1), their preconditions (2) and effects (3) as well as the type hierarchy (4).}
        \label{fig:nl_domain}
    \end{subfigure}
    \caption{Excerpts from the typed (top) and untyped (bottom) version of the PDDL Logistics domain definition (\ref{fig:pddl_domain}) and the NL domain description generated by \resourcename\ (\ref{fig:nl_domain}).}
    \label{fig:domain_ex}
\end{figure*}
\end{comment}


\section{Background}\label{sec:rel_work}

PDDL \cite{pddl1998ghallab} has been established in the context of the
International Planning
Competitions\footnote{\url{https://www.icaps-conference.org/competitions/}}.
A planning task in PDDL consists of a domain and problem file.
The domain file defines the world model using predicates describing
possible world states, and actions whose execution changes the current state.
The problem file defines a specific instance from the domain by specifying
available objects, the initial state and the goal.

Each action is defined by its precondition specifying what has to be true
in the state where the action is applied, and by its effect saying what
will become true (add effect) and false (delete effect) in the resulting
state.
The solution to a planning problem is a plan---a sequence of actions
leading from the initial state to a state where the goal condition holds.

Figure~\ref{fig:pddl_domain} shows an excerpt from the Logistics benchmark domain
that models delivering packages with trucks within cities and with
planes between cities. % until each package is at its goal location.
The action ``drive-truck'' describing driving a truck between two locations
is parametrized with variables
``?truck'', ``?loc-from'', ``?loc-to'' and ``?city'' whose
instantiation with objects specifies the truck being driven, the start and
the destination location and the city in which the locations are.
The precondition states that the action can only be executed if the truck
is at location ?loc-from and both locations are in city ?city.
The effect makes the atom (at ?truck ?loc-from) false and (at ?truck
?loc-to) becomes true, i.e., it changes the state by moving the truck
?truck from ?loc-from to ?loc-to.

Variables can also have types restricting which objects can be used for
their instantiation.
For example, ?truck has the type ``truck'' which in our example
has only one corresponding object ``t0''.
%
There are different variants of the PDDL language with varying
expressiveness.
Here, we consider a PDDL subset allowing variable typing and
restricted to conjunctive conditions with negation.


\begin{figure*}[t]
    \centering
    \subfloat[PDDL domain definition with the type hierarchy ($\mathcal{T}$), predicates ($\mathcal{P}$), and the ``drive-truck'' action ($\mathcal{A}$).]{\includegraphics[width=0.35\textwidth]{pictures/pddl_domain_typed.pdf}\label{fig:pddl_domain}}
    \qquad
    \subfloat[NL domain description consisting of the available actions with parameters ($\mathcal{A^{PA}}$), their preconditions ($\mathcal{A^{PR}}$) and effects ($\mathcal{A^E}$) and the type hierarchy ($\mathcal{T}$).]{\includegraphics[width=0.55\textwidth]{pictures/nl_domain_ex.pdf}\label{fig:nl_domain}}
    
    \subfloat[PDDL problem file stating the available objects with types ($\mathcal{O}$), the initial state ($\mathcal{I}$) and the goal condition ($\mathcal{G}$).]{\includegraphics[width=0.35\textwidth]{pictures/pddl_problem.pdf}\label{fig:pddl_prob}}
    \qquad
    \subfloat[NL problem description stating the goal ($\mathcal{G}$), the available objects ($\mathcal{O}$) and the initial state ($\mathcal{I}$).]{\includegraphics[width=0.55\textwidth]{pictures/problem_nl.pdf}\label{fig:nl_problem}}
    \caption{\label{fig:domain_ex}%
Part of the Logistics PDDL domain %(\ref{fig:pddl_domain})
and problem %(\ref{fig:pddl_prob})
file and the NL descriptions generated by {\resourcename}. %(\ref{fig:nl_domain}, \ref{fig:nl_problem}).
}
\end{figure*}


\begin{comment}
\begin{figure}[t]
    \centering
    \subfloat[PDDL domain definition with the type hierarchy ($\mathcal{T}$), a subset of predicates ($\mathcal{P}$), and the ``drive-truck'' action ($\mathcal{A}$).]{\includegraphics[width=0.48\textwidth]{pictures/pddl_domain_typed.pdf}\label{fig:pddl_domain}}
        
    \par\bigskip
    \subfloat[PDDL problem file consisting of the available objects with their types ($\mathcal{O}$), the initial state ($\mathcal{I}$) and the goal condition ($\mathcal{G}$).]{\includegraphics[width=0.48\textwidth]{pictures/pddl_problem.pdf}\label{fig:pddl_prob}}
    \caption{Excerpt from the typed PDDL Logistics domain definition (\ref{fig:pddl_domain}) and an example problem file (\ref{fig:pddl_prob}).}
    \label{fig:domain_ex}
\end{figure}
\end{comment}

%The Planning Domain Description Language (PDDL) \cite{pddl1998ghallab} is a popular language to encode classical planning problems used also in the International Planning Competitions\footnote{\url{https://www.icaps-conference.org/competitions/}}. PDDL planning tasks consist of a domain file and a problem file. Figure \ref{fig:domain_ex} presents an excerpt of the domain file (top) and a problem file from the Logistics domain where the task is to transport packages with trucks within cities and with planes between cities until each package is at its goal location.
%
%The domain file encodes the definition of the world model including the actions that can be executed and the predicates defining the possible world states.   
%The action ``drive-truck'' has four parameters ``?truck'', ``?loc-from'', ``?loc-to'' and ``?city'' that are variables for actual objects that correspond to the truck being driven, the start and the destination location and the city in which the locations are. The preconditions specify that the action can only be executed if the truck is at the ?loc-from location and both locations are in the specific city. The effect of an action defines how the action changes the world state. For example, driving the truck from the start to the destination location has the effect that the predicate (at ?truck ?loc-from) is no longer true and (at ?truck ?loc-to) becomes true.
%
%For each action parameter the type constraints are specified, e.g. ``?truck'' needs to be an object of type ``truck''. The type definitions are optional in PDDL and untyped domains include them in the form of unary predicates in the preconditions. % type constraints in the form of unary predicates in the action preconditions instead (e.g. ``(truck ?truck)'').
%%In the untyped version shown at the bottom unary predicates, such as (truck ?truck), are included as preconditions to ensure that the actions are applied only to appropriate kinds of objects.
%
%A problem file defines a specific instance of a problem from a domain and specifies the available objects, the initial state and the goal. The initial state is defined in terms of all state predicates that are true at the beginning and the goal is a set of predicates that need to become true. A plan for the problem corresponds to a sequence of actions that will change the world state from the initial state to a world state satisfying the goal conditions.  
%
%There exist different versions of the PDDL language that vary with regard to their expressiveness. In the current work, we focus on domains that contain only ``and" and ``not" as operators and do not include action costs or numeric values. Our approach considers both typed and untyped domains. 


\paragraph{PDDL and LLMs.}

%\citet{valmeekam2023planbench} presented Planbench, a benchmark framework for assessing different aspects of the reasoning capabilities of LLMs based on classical planning problems formulated in PDDL. They provide a suite of test cases including plan generation, optimal planning and reasoning about execution. Their framework automates the generation of natural language (NL) state descriptions, plans and of test case specific few-shot examples. Their approach requires the existence of textual descriptions of the domains to be tested and for the generation of the NL descriptions of problems, objects and plans they rely on manually created templates for mapping actions and predicates into NL fragments. 

%Overall, their assessment pipeline first translates actions, predicates and state descriptions from PDDL to NL. Then, an LLM is prompted to generate a plan based on a description of the domain, the automatically generated NL descriptions of the initial and goal state and the few-shot examples. In the last step, the predicted NL plans get translated into PDDL to automatically evaluate them using a plan validator. This automation of the assessment process allows a systematic and objective evaluation of the performance of LLMs on different reasoning related test cases. 

\citet{valmeekam2023planbench} introduced Planbench, a benchmark framework for assessing different aspects of reasoning capabilities of LLMs based on classical planning problems formulated in PDDL. Their assessment pipeline can take PDDL domain and problem files as input as well as natural language (NL) descriptions of the PDDL domain and problem files for assessing LLMs on NL problem formulations. 
For the NL inputs, they manually create a NL description of the domain file and handcraft NL translations for the individual PDDL actions, predicates and for object names. The individual translations are used to compose NL descriptions of problem files and plans. 

In their assessment pipeline, \citet{valmeekam2023planbench} prompt an LLM to generate a plan based on the NL descriptions of the domain, the initial and goal state and few-shot examples, i.e., example problems with their corresponding plans for in-context learning. The predicted NL action sequences get translated back into PDDL by a domain-dependent translator  and are automatically evaluated by a plan validator. This process allows a systematic and objective evaluation of the performance of LLMs on different reasoning-related test cases.
However, the approach includes several manually provided per-domain components. 
%
% Joerg: the larger benchmark basis no longer is our main point; maual input is bad enough on its own
%
%Extending the framework to new domains in addition to the three domains %provided by \citet{valmeekam2023planbench} requires manual effort such as the %creation of all NL descriptions for the target PDDL domain.
%the approach requires manual effort for extending the assessment beyond the three domains for which \citet{valmeekam2023planbench} provide them. Additionally, they rely on manually created mappings from PDDL actions and predicates to NL fragments to generate NL encodings of the problem files as well as domain-dependent translation components for translating the NL output back into PDDL action sequences. 

\citet{silver2022pddl} assess the planning capabilities of LLMs when using prompts that do not contain any natural language and consist of the target problem definition and two few-shot examples in PDDL. They evaluate OpenAI's Codex LLM \cite{codex}, an LLM specifically trained to generate code for NL inputs, and find that in some domains such as Gripper and Movie, LLMs can solve even large problems while they completely fail on more than half of the evaluated domains, including Blocksworld.

\citet{valmeekam2023planning} also assess the LLM capabilities on PDDL but their prompts include a general task description in NL and the PDDL domain in addition to the target problem and examples.
% Joerg: unnecessary detail
%They find that for Blocksworld, using PDDL inputs leads to a drop in %performance compared to NL whereas on Logistics they do not observe %differences.
%
Recent work explored the generation of Python code representing per-domain generalizing action policies \cite{silver2024generalized}.
%
There has also been works investigating the use of LLMs as an interface between problems in NL and symbolic AI planning tools.
%to obtain PDDL representations for natural language planning problems and plans. 
\citet{liu2023llmp} propose to use LLMs to translate NL descriptions of planning problems into PDDL. They then use a symbolic planner to find a plan and translate that back into NL. \citet{xie2023translating} use LLMs to translate NL goals into PDDL. % goal definitions. 


